Towards Building Self-Aware Object Detectors via Reliable Uncertainty Quantification and Calibration

The current approach for testing the robustness of object detectors suffers from serious deficiencies such as improper methods of performing out-of-distribution detection and using calibration metrics which do not consider both localisation and classification quality. In this work, we address these issues, and introduce the Self-Aware Object Detection (SAOD) task, a unified testing framework which respects and adheres to the challenges that object detectors face in safety-critical environments such as autonomous driving. Specifically, the SAOD task requires an object detector to be: robust to domain shift; obtain reliable uncertainty estimates for the entire scene; and provide calibrated confidence scores for the detections. We extensively use our framework, which introduces novel metrics and large scale test datasets, to test numerous object detectors in two different use-cases, allowing us to highlight critical insights into their robustness performance. Finally, we introduce a simple baseline for the SAOD task, enabling researchers to benchmark future proposed methods and move towards robust object detectors which are fit for purpose. Code is available at https://github.com/fiveai/saod

==> Sections/1.Introduction-2.tex <==
\section{Introduction}\label{sec:introduction}
%
\begin{figure}[ht]
        \centering
        \includegraphics[width=0.48\textwidth]{Images/Teaser.pdf}
        \caption{(Top) The vanilla object detection task vs. (Bottom) the self-aware object detection (SAOD) task. Different from the vanilla approach; the SAOD task requires the detector to: predict $\hat{a} \in \{0,1\}$ representing whether the image is accepted or not;  discard noisy detections (see bike images); and be evaluated on clean ID, corrupted ID and OOD images using our DAQ measure.
        }
        \label{fig:teaser}
\end{figure}
%
%
%The task of object detection requires a model to localize objects in an image by surrounding them with a bounding box and assigning each of them one out of $K$ pre-determined classes, aka in-distribution (ID) classes or objects. 
%
Object detectors are particularly common in safety-critical applications such as autonomous driving \cite{Cityscapes,bdd100k,waymo}.
%
As such, the safe and reliable usage of an object detector depends not only on its accuracy, but also critically on other performance aspects, such as its ability to obtain well-calibrated predictions and to flag a scene for human intervention when it is uncertain, a process termed rejection.
%confidence is below a pre-determined threshold and flag the image for human intervention.
%
Therefore, during their development it is essential to have a thorough evaluation framework including such robustness aspects.
%
In this work we propose such a framework; specifically our framework evaluates the reliability of the uncertainties, robustness to domain shift, calibration and accuracy of object detectors in unified and principled manner.

Current evaluation methodologies that consider robustness aspects of object detectors have notable drawbacks. 
%
Firstly, the evaluation is conducted on small-scale test sets and without a validation (val) set.
%
To illustrate, recent works \cite{RegressionUncOD,VOS} leverage out-of-distribution (OOD) detection as a proxy task to evaluate the reliability of the uncertainties following the classification literature \cite{DUQ,DDU,regmixup}.
%
However, the proposed OOD test sets in this context only have around 1-2K images, limiting the thoroughness of the evaluation. 
%
Moreover, as val sets are typically unavailable, practitioners are forced to use unideal solutions to tune the hyper-parameters, such as relying on the training set \cite{devil,Norcal}, directly using the test set \cite{RegressionUncOD,VOS} or splitting the test set in two, further reducing its size \cite{mvcalibrationod}. 
%
%\textbf{(D2)} \emph{OOD detection at the detection-level is non-trivial, as conceptually there is no clear definition as to which detections can be considered ID and which cannot; despite this, previous work ~\cite{RegressionUncOD,VOS} seek to label individual detections as OOD or ID.}
%
%To elaborate further, unknown objects may appear in two forms at test time.
%
%Namely, they may appear as ``known-unknowns'', which can manifest as background and unlabelled objects in the training set. 
%
%However, they can also appear as ``unknown-unknowns'', completely unseen objects, which are not present in the training data.
%
%It is not possible to split these unknown objects into the two categories without having labels for every pixel in the training set~\cite{opensetelephant}.
%
%Current evaluation \cite{RegressionUncOD,VOS} however, does not adhere to this structure and instead defines ``an image'' with no ID object as OOD but assumes ``any detection'' in an OOD image is an OOD detection, and vice versa for an ID image.
%
%This approach completely disregards the nuances of the situation at hand, which as shown in Fig. \ref{fig:teaser}(a) is a scenario which occurs frequently.
%
% \textbf{(D3)} Existing calibration measures for object detection \cite{CalibrationOD,mvcalibrationod} focus on either classification or localization, but not both, ignoring the implicitly joint nature of object detection.
%
Last but not the least, methods typically focus on either accuracy \cite{KLLoss,sampleweightingnet,BayesOD}; classification calibration~\cite{CalibrationOD}; localisation calibration ~\cite{mvcalibrationod}; OOD detection~\cite{VOS}; or domain-shift~\cite{RobustnessODBenchmark,oddomainshiftcycle}, with no prior work taking a holistic approach by evaluating all of them.

In this paper, we provide a framework to evaluate object detectors thoroughly also by addressing the aforementioned deficiencies:
%
Specifically our contributions are as follows.

\textbf{(C1)} We first construct new test sets comprising in-distribution (ID) images with domain shift and OOD images for two different settings: General object detection (Gen-OD) and autonomous vehicle object detection (AV-OD). 
%
Our test sets are significantly larger (i.e. 45K for each ID set and 110K for the OOD set) and do not include any images from the val sets, thereby  properly allowing them to be used for hyper-parameter tuning.

\textbf{(C2)} We introduce image-level uncertainties to enable an object detector for rejecting an entire scene when it is uncertain.
%
%OOD detection at the image-level, thereby aligning the evaluation with the definition.
%
For this, we propose and comprehensively evaluate several methods for obtaining image-level uncertainties using a wide range of detectors.
%
Our analysis suggests that object detectors inherently yield reliable image-level uncertainties and provide the crucial functionality to reject images with high uncertainty (Fig. \ref{fig:teaser}(a)).

\textbf{(C3)}
%
We provide a principled definition of calibration error for object detectors, termed the mean ECE (mECE), which faithfully accounts for the joint nature of object detectors by considering both classification and localisation.

\textbf{(C4)}
%
Finally, we design the novel self-aware object detection (SAOD) task, which requires the detectors to (i) be robust against domain shift; (ii) obtain reliable image-level uncertainty estimates; (iii) be accurate; and (iv) yield calibrated detections (Fig. \ref{fig:teaser}(b)). 
%
We further propose the Detection Awareness Quality (DAQ) which considers these requirements in a unified manner and also propose a baseline to convert any object detector into one that is self-aware.
%



==> Sections/1.Introduction.tex <==
\section{Introduction}\label{sec:introduction}
%
\begin{figure*}[ht]
        \captionsetup[subfigure]{}
        \centering
        \begin{subfigure}[b]{0.26\textwidth}
        \includegraphics[width=\textwidth]{Images/Images.pdf}
        \caption{ID vs. OOD image from \cite{VOS}}
        \end{subfigure}
        \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[width=\textwidth]{Images/corruption.pdf}
        \caption{Using image-level uncertainties}
        \end{subfigure}
        \begin{subfigure}[b]{0.40\textwidth}
        \includegraphics[width=\textwidth]{Images/Teaser.pdf}
        \caption{Object detection vs. self-aware object detection.}
        \end{subfigure}
        \caption{\textbf{(a)} ID and OOD images taken from the test set in \cite{VOS}. Both contain objects of class ``flag'' (in red rectangles), which is not one of the ID classes. Hence, it is not trivial to label detections as ID or OOD in detection-level. Instead, we evaluate methods in image-level. \textbf{(b)} A use-case of image-level uncertainties obtained from Faster R-CNN (Gen-OD) based on our analysis. As the severity of corruption increases, less images are accepted by the detector. Also, the performance of the rejected images is notably lower than that of accepted images. These, both, imply the reliability of the uncertainties. Supp.Mat. shows that this is consistent across detectors. \textbf{(c)}  Object detection (OD) vs. self-aware object detection (SAOD). Different from OD; SAOD (i) is tested not only on ID images, but also on corrupted and OOD images, (ii) requires $\hat{a} \in \{0,1\}$ representing whether the image is accepted or not, (iii) requires properly thresholded detections (compare example output images of OD and SAOD) and (iv) relies on DAQ for evaluation, combining OOD detection, accuracy, calibration and robustness to corruptions. Blue: Our additions to object detection, red: SAOD removes top-k and requires properly-thresholded detections.}
        \label{fig:teaser}
\end{figure*}
%
%
The task of object detection requires a model to localize objects in an image by surrounding them with a bounding box and assigning each of them one out of $K$ pre-determined classes. 
%
The use cases of such detectors varies significantly, but they are particularly common in safety-critical applications such as autonomous vehicles (AV) \cite{Cityscapes,bdd100k,waymo}.
%
As such, the safe and reliable usage of these detectors depend not only on their accuracy, but also critically on other performance aspects, such as their ability to obtain well calibrated predictions and reject images if the confidence is below a pre-determined threshold and flag the image for human intervention.
%
Consequently, it is essential to have a carefully designed and thorough evaluation framework which considers all of these performance aspects.
%
In this work we propose such a framework; specifically our framework evaluates the reliability of uncertainties, robustness to domain shift, calibration and accuracy of object detectors in unified and principled manner.

Current evaluation methodologies wrt. robustness aspects for object detectors have notable drawbacks:
%
\textbf{(D1)} \textit{The evaluation is conducted on small-scale test sets and without a validation (val) set.}
%
To illustrate; recent works \cite{RegressionUncOD,VOS} leverage OOD detection as a proxy task to evaluate the reliability of the uncertainties following classification \cite{DUQ,DDU,regmixup}.
%
However, proposed OOD datasets in this context only have around $1K - 2K$ images, limiting the thoroughness of the evaluation. 
%
Moreover, as val sets are typically unavailable, practitioners are forced to use unideal solutions to tune the hyper-parameters, such as relying on training set \cite{devil,Norcal}, directly using the test set \cite{RegressionUncOD,VOS} or splitting the test set in two, further reducing its size \cite{mvcalibrationod}. 
%
\textbf{(D2)} \textit{Current evaluation \cite{RegressionUncOD,VOS} of OOD detection aims to label detections as ID or OOD, however, this is conceptually non-trivial for object detection.}
%
This is because each pixel is not labeled in the detection datasets.
%
Specifically, unknown objects may appear in both ID and OOD images either as a ``known-unknown'', background and undesired objects in the training set or as an ``unknown-unknown'', a completely unseen object; and it is not possible to split unknown objects into those categories without labelling every pixel \cite{opensetelephant}.
%
%Besides, splitting objects as known-unknowns or unknown-unknowns is not possible, giving rise to ``mixed-unknowns'' as discussed by Dhamija et al.
%in addition to objects from ID classes (``known-known''); a detector may face (i) an object that is among background (``known-unknown'') in the training set, hence to be rejected, or (ii) a completely unseen object (``unknown-unknown'').
%
%Since not each pixel is not labeled in object detection datasets, it is not possible to split objects as known-unknowns and unknown-unknowns, giving rise to ``mixed-unknowns'' as discussed by Dhamija et al. \cite{opensetelephant}.
%
%However, for object detection
% Unlike classification which operates at the image level, discriminating between ID and OOD is non-trivial for object detectors.
%
%This is due to the conceptual difficulty of labelling the detections as ID or OOD at the object level.
%
%There are three sets of classes: \emph{known-knowns} (1 of $K$), \emph{known-unknown} (background objects from training data); and \emph{unknown-unknowns} (objects which the classifier has never seen before).
%
% Note convolute, between image level and detection level, in detection level it is wrong
%
Current evaluation \cite{RegressionUncOD,VOS} defines  ``an image'' with no ID object as OOD but assumes ``any detection'' originating from an OOD (ID) image is an OOD (ID), disregarding the nuances of the situation at hand.
%
Thus, unknown objects with the same semantic category commonly appear in both ID or OOD images as ``flag'' in Fig. \ref{fig:teaser}(a), decreasing the reliability of the evaluation.
%
%
% as objects which are assigned a background class in the training data may infact be present in the supposed OOD set.
%However, 
% Existing approaches neglect the presence of the known-unknowns~\cite{RegressionUncOD,VOS}, and define an image with no ID object as OOD.
%
%
%This can be seen in Fig. \ref{fig:teaser}, where the ``flag'' is present on both the ID image, and the OOD image, i.e., a ``mixed unknown'' as defined in \cite{opensetelephant}.
%
%In this situation, the ``flag'' is in fact ID, although the methodology does not treat it as such.
%
% Labeling ``detections'' as ID or OOD, which is the existing approach for OOD evaluation \cite{RegressionUncOD,VOS}, is not trivial for object detection.
% %
% This is because the behaviour of the object detector can vary depending whether an object, that does not pertain to ID classes, is included in the background of the training set (see ``flag'' in Fig. \ref{fig:teaser}(a)), i.e., a ``mixed unknown'' as defined by Dhamija et al. \cite{opensetelephant}:
% %
% If such an object is included in the training set (``known unknown''), the detector can reject them; else it is ``unknown unknown'' and can be detected both in ID and OOD images as one of the ID classes.
% %
% Current evaluation defines an OOD image as \textit{an image with no ID objects} and assumes any detection originating from an OOD (ID) image is an OOD (ID) detection.
    % %
    % However; this assumption ignores mixed unknowns and it is not aligned with definition of OOD data which is in image-level.
    % %
    % Besides, underlying ground-truth objects are not considered at all, implying any false positive detection to be labelled as ID or OOD according to the image that it belongs to.
    %
\textbf{(D3)} \textit{Existing calibration measures for object detection \cite{CalibrationOD,mvcalibrationod} focus on either classification or localization, but not both, ignoring the joint nature of object detection.}
%
To illustrate, Detection ECE \cite{CalibrationOD} aims to align confidence scores only with precision, thereby mainly considering classification.
%
%and Kuppers et al. \cite{mvcalibrationod} focus solely on calibration of localization task for probabilistic detectors.
%
\textbf{(D4)} \textit{The methods are evaluated either wrt. mainly accuracy \cite{KLLoss,sampleweightingnet,BayesOD} or some robustness aspects, but only partially.} 
%
As examples to the latter; while VOS \cite{VOS} does not consider domain shift or calibration but delve into OOD detection, some works \cite{RobustnessODBenchmark,oddomainshiftcycle} only focus on domain shift.
%
%

%, the reliability of uncertainties is evaluated in detection-level by assuming that any detection originating from an OOD (ID) image is an OOD (ID) detection, ignoring mixed unknowns.
%
% However, \textit{(D2) labeling detections as ID or OOD is not trivial for object detection} since only ID objects are annotated in the datasets and an unannotated object from the same class may appear both in ID and OOD images (e.g., see ``flag'' objects in Fig. \ref{fig:teaser}(a)). 
%
% As a result, the expected behaviour of the object detector vary depending whether such objects are included in the background of the training set, which are defined as ``mixed unknowns'' by Dhamija et al. \cite{opensetelephant}:
%
% If such an object is included in the training set (known unknown), the detector can reject them; else the object is unknown unknown and can be detected both in ID and OOD images to one of ID classes. 
%
% As a result, labelling detections depending solely on the image they originate may not provide a reliable evaluation of uncertainty scores.
%

%

%

%However, this has not take much attention and some bad practices are commonly used in the literature.
%
%First, the reliability of the uncertainties is evaluated based on very small datasets. 
%
%For example, a recently proposed dataset, designed for OOD detection for object detection, has 4952 Pascal VOC \cite{PASCAL} images as in-distribution (ID) data and a subset of COCO \cite{COCO} with only 930 images as OOD data.
%
%Second, some proposed datasets \cite{RegressionUncOD,VOS} do not have a hold-out validation set and some \cite{COCO,LVIS,nuimages} do not provide the annotations of the test set. 
%
%These resulted in different unideal solutions for cross-validating the hyperparameters.
%
%Some methods \cite{mvcalibrationod} split test set into two, further reducing the dataset size; others (e.g., NorCal \cite{Norcal}) use training set to tune hyperparameters and a third group tune hyperparameters on the test set (e.g., VOS \cite{VOS} obtains detection confidence score threshold using optimal f-score computed on ID test set).
%
%Last but not the least, it is not trivial to label the detections as ID or OOD since only a small subset of the possible object classes are annotated in object detection.
%
%Hence, it may not be a valid assumption to consider all detections from an ID test image are ID and those from an OOD test image are OOD (Fig. \ref{fig:teaser}(a)), which is yet another convention \cite{VOS}. 
%

%Existing studies \cite{unc_est_safety_critical,unc_est_merging,BayesOD,KLLoss,RegressionUncOD,VOS,OWOD,OW-DETR,UC-OWOD,sampleweightingnet} focus heavily on obtaining reliable detection-level uncertainty and almost ignored image-level uncertainty. 
%
%It has been shown that the detector can benefit from detection-level uncertainties in several ways: They can be used for weighting the examples in the loss function \cite{sampleweightingnet}, for better Non-Maximum-Suppression strategies \cite{KLLoss,BayesOD}, for out-of-distribution (OOD) detection and for identification of novel objects \cite{VOS,OWOD,OW-DETR,sampleweightingnet}.  
%
%As for image-level uncertainty estimation; as a notable work, Choi et al.\cite{ActiveLearningOD} leveraged them for active learning in object detection. 
%
%However, other potential benefits of image-level uncertainty estimations still remain unexplored.

% In this paper, 

% Overall, (i) these works focus an individual aspect of robustness (covariate shift, reliable uncertainty estimation and calibration) with some \cite{RegressionUncOD,KLLoss} focusing on a single task (e.g. localization) for a particular robustness aspect, (ii) none of them computes uncertainty in the image-level, which potentially, can provide the overall reliability of an object detector for a given scenario and (iii) for evaluation, they commonly employ validation set, which, generally, comprises a small number of images, includes only in-distribution (ID) data and used for cross-validating hyper-parameters.
%
In this paper, we address the aforementioned deficiencies and provide a framework to evaluate object detectors thoroughly. 
%
To do so; we make four contributions, each of which addresses a drawback of existing evaluation methodology.
%
\textbf{(C1)} We first construct new test sets comprising ID images with domain shift and OOD images for two different settings: General object detection (Gen-OD) and AV object detection (AV-OD). 
%
Our test sets are significantly larger (i.e. 45K for each ID and 110K for OOD) and do not include any image from val sets, thereby  properly allowing them to be used for hyper-parameters tuning.
%
\textbf{(C2)} We rely previous work \cite{VOS,RegressionUncOD} to define an OOD image (i.e., an image without an ID object), but differently, we require a detector to reject images (not the detections), thereby aligning the evaluation with the definition.
%
We propose and comprehensively evaluate several methods for obtaining image-level uncertainty using a diverse set of object detectors.
%
Our analysis suggests that object detectors are, in fact, very strong OOD detectors and this provides the crucial functionality to reject images with high domain shift (Fig. \ref{fig:teaser}(b)).
%   
%Noting that using image-level uncertainties is not common in object detection\footnote{To the best of our knowledge, the only use case of image-level uncertainties is for active learning in object detection\cite{ActiveLearningOD}}, we comprehensively analyse how to obtain reliable image-level uncertainties using a diverse set of object detectors.
%
%Our analysis suggests that object detectors are, in fact, very strong OOD detectors and the resulting uncertainties can be leveraged to reject images with high domain shift (Fig. \ref{fig:teaser}(b)).
%
\textbf{(C3)} We provide a robust definition of calibration error for object detectors (mECE) which faithfully accounts for the joint nature classification and localisation performance.
%
%We derive mean Expected Calibration Error (mECE) for object detection.
%
%Unlike existing measures \cite{CalibrationOD,mvcalibrationod}; mECE considers the joint nature of object detection, thereby measuring the disparity of confidence not only with classification performance, but also with localization performance.
%
%We analyze how calibration and accuracy measures should be coupled and investigate standard baselines for calibration.
%
\textbf{(C4)} 
Finally, we design novel self-aware object detection (SAOD) task, which permits the detectors to reject images if they are uncertain.
%
Specifically, SAOD requires the detectors to (i) be robust against domain shift, (ii) obtain reliable uncertainty estimation, (iii) be accurate and (iv) yield calibrated detections (Fig. \ref{fig:teaser}(c)). 
%
We further propose Detection Awareness Quality (DAQ) to measure the performance of the SAOD methods and a baseline to convert any object detector to a self-aware one.
%and provide large scale datasets, consisting of domain shift and OOD data for general object detection and autonomous driving problems.
%    
%Finally, we design self-aware object detection (SAOD) as a novel detection task. 
%
%SAOD requires the detectors to (i) be robust against domain shift, (ii) obtain reliable uncertainty estimation, (iii) be accurate and (iv) yield calibrated detections (Fig. \ref{fig:teaser}(c)). 
%
%We propose Detection Awareness Quality (DAQ) to measure the performance of methods on SAOD task and propose a baseline to convert any object detector to a self-aware one.
%

\blockcomment{
%
\begin{itemize}
    \item We propose and comprehensively evaluate several methods for obtaining image level uncertainty from the output of a diverse object detectors.
    %
    Our analysis suggests that object detectors are, in fact, very strong OOD detectors and this provides the crucial functionality to reject images with high domain shift (Fig. \ref{fig:teaser}(b)).
    %
    \item We provide a robust definition of calibration error for object detectors (mECE) which faithfully accounts for the joint nature of classification and localisation performance.
    %
    %We further define ID Quality (IDQ), which provides a measure on how in distribution a sample is. 
    %
    %The metric decomposes as the harmonic mean of localization accuracy, classiciation performance and mECE.
    %
    \item Finally, our main contribution is the design of the novel self-aware object detection (SAOD) task, which permits object detectors to reject images if they are uncertain.
    %
    Specifically, SAOD requires the detectors to (i) be robust against domain shift, (ii) obtain reliable uncertainty estimation, (iii) be accurate and (iv) yield calibrated detections (Fig. \ref{fig:teaser}(c)). 
    %
    To evaluate the models we propose Detection Awareness Quality (DAQ) which measures the performance of the methods.
    %
    We further propose a baseline to convert any object detector to a self-aware one and provide large scale datasets, consisting of domain shift and OOD data for general object detection and autonomous driving problems.
    
    % \item \textbf{(C1)} We rely on the definition of an OOD image (i.e., an image without an ID object) of previous work \cite{VOS,RegressionUncOD}, but differently, we require a detector to reject images (not the detections), thereby aligning the evaluation with the definition.
    % %
    % Noting that using image-level uncertainties is not common in object detection\footnote{To the best of our knowledge, the only use case of image-level uncertainties is for active learning in object detection\cite{ActiveLearningOD}}, we comprehensively analyse how to obtain reliable image-level uncertainties using a diverse set of object detectors.
    % %
    % Our analysis suggests that object detectors are, in fact, very strong OOD detectors and the resulting uncertainties can be leveraged to reject images with high domain shift (Fig. \ref{fig:teaser}(b)).
    %
    % \item \textbf{(C2)} We derive mean Expected Calibration Error (mECE) for object detection.
    % %
    % Unlike existing measures \cite{CalibrationOD,mvcalibrationod}; mECE considers the joint nature of object detection, thereby measuring the disparity of confidence not only with classification performance, but also with localization performance.
    %
    % We analyze how calibration and accuracy measures should be coupled and investigate standard baselines for calibration.
    %
    % \item \textbf{(C3)} Finally, we design self-aware object detection (SAOD) as a novel detection task. 
    % %
    % SAOD requires the detectors to (i) be robust against domain shift, (ii) obtain reliable uncertainty estimation, (iii) be accurate and (iv) yield calibrated detections (Fig. \ref{fig:teaser}(c)). 
    % %
    % We propose Detection Awareness Quality (DAQ) to measure the performance of methods on SAOD task and propose a baseline to convert any object detector to a self-aware one.
    % %
    % \item \textbf{(C4)} We first construct new test datasets comprising of ID data with domain shift and OOD data under two different settings: General object detection (Gen-OD) based on COCO \cite{COCO} and autonomous vehicle object detection (AV-OD) based on nuImages \cite{nuimages}. 
    % %
    % Our test datasets are significantly larger in scale (i.e. 45K for each ID and 110K for OOD) and do not include any image from COCO or nuImages val sets, enabling the val sets to be used for proper tuning of hyper-parameters.

\end{itemize}
}
%

%

%
%As a result, we address the aforementioned drawbacks (D1-D3) of the existing works.
%
\blockcomment{
Our main contributions are summarized as follows: 
%
\begin{compactitem}
    %
    \item We present two new test datasets for Gen-OD and AV-OD, each of which comprising ID data with domain shift and OOD data.
    %
    To the best of our knowledge, this is the first work to include a large-scale OOD dataset for object detection task.
    %
    \item We provide a comprehensive analysis to obtain reliable image-level uncertainty using a diverse set of object detectors and discover that object detectors are, in fact, very strong OOD detectors.
    %
    In particular, we show that various object detectors consistently reject SVHN cropped digits \cite{SVHN}, currently a very common OOD baseline for classifiers \cite{DUQ,DDU,regmixup}, with $99.9$ AUROC score, i.e. almost perfect performance.
    %
    \item We derive mean Expected Calibration Error (mECE) for object detection.
    %
    Different from existing measures, mECE focuses on the disparity of confidence not only with classification performance, but also with localization performance.
    %
    \item We devise self-aware object detection task, considering various robustness aspects. 
    %
    For this new task, we propose (i) Detection Awareness Quality as a performance measure considering domain shift, accuracy, calibration and OOD detection in a unified manner and (ii) a baseline to convert any object detector to a self-aware object detector.
\end{compactitem}
}

% fills that important gap by collecting test sets (Section \ref{sec:dataset}), exploring uncertainty estimation (Section \ref{sec:ood}), defining calibration from a joint perspective of classification and localization (Section \ref{sec:calibration}) and proposing self-aware object detection task to facilitate research in this direction (Section \ref{sec:evaluation}) 
%
%
%The ability to detect objects within an image, assign a bounding box and predict their class is an critical feature needed for autonomous systems such as self driving cars.
%
%Despite their wide range of applications, there is a critical gap in the literature which comprehensively exams their robustness.
%
%Existing limited research focuses generally on a single aspect of an object detectors robustness such as calibration \cite{CalibrationOD,mvcalibrationod} or detection-level uncertainty estimation \cite{RegressionUncOD, VOS}. 
%
% Up until this point, evaluating the robustness of object detectors has mainly been limited by the absence of the necessary tools, such as: reliable object-level uncertainty estimation techniques; representative datasets; and evaluation measures.
%
% In this paper we address these shortcoming in the literature by developing a framework to effectively evaluate the robustness of object detectors.
%

% \paragraph{What is OOD in object detection?} 
%
\blockcomment{
\subsection{Related Work}
%
\paragraph{Uncertainty Estimation in Object Detection} Most of the works focused on obtaining reliable uncertainties in the detection-level. 
%
Earlier methods \cite{unc_est_safety_critical,unc_est_merging} show that reliable detection uncertainties can be obtained using Monte-Carlo dropout.
%
A group of works \cite{BayesOD,KLLoss} represent the box locations by Gaussian distribution and optimizing negative log likelihood (NLL) to learn the Gaussian distribution. 
%
This optimization is shown to be effective and leveraging the covariance of the Gaussian distribution for postprocessing improve accuracy of the models.
%
A different study \cite{sampleweightingnet} uses the predicted covariance and the uncertainty of the classifier to weight the samples in the loss function during training.
%
None of these methods have not considered uncertainties from robustness perspective but focus mainly on improving the accuracy.
%
Recently, Harakeh and Waslander \cite{RegressionUncOD} show that optimizing energy score is a better alternative to NLL to capture the localization uncertainty.
%
VOS \cite{VOS} synthesizes virtual outliers to supervise the model to distinguish ID and OOD detections.
%
VOS discards the noisy detections by tuning the optimal threshold on test set based on optimal f-score, which is not feasible in a practical application.
%
It is also assumed that any detections obtained in the ID test set are ID and those in the OOD test set are OOD.
%
However, ID test data can include several objects not pertaining to ID classes, which may affect the reliability of the evaluation.
%
These recent works \cite{RegressionUncOD,VOS} relying on detection-level uncertainty estimation also present OOD datasets with a size generally around $1-2k$ images, which is limited for a thorough evaluation of the models. 
%
Open-world object detectors \cite{OWOD,OW-DETR,UC-OWOD}, as a related set of methods, aim to identify unknown objects and learn them after explicit labelling without forgetting the previous classes, thereby requiring detection-level uncertainty.
%
Instead of computing detection-level uncertainty, Choi et al. \cite{ActiveLearningOD} leveraged image-level uncertainty for active learning, which has been shown to be useful for that particular task.
%
\paragraph{Calibration of Object Detectors}
%
While object detection in a joint task of classification and localization, current approaches focus on a single aspect in terms of calibration.
%
Detection ECE \cite{CalibrationOD} measures the misalignment between precision for a specific true positive threshold and accuracy, thereby focusing on classification.
%
In order to provide spatial analysis, the authors also discretize the image-space into grids, however they do not compare the confidence of an object detector with its localization performance.
%
Conversely, a different work \cite{mvcalibrationod} aims to calibrate the localization head of the probabilistic detectors, without considering the resulting detection score.
%
\paragraph{Covariate Shift in Object Detection}
%
This aspect of robustness has not been thorougly considered.
%
As an important work, Michaelis et al. \cite{RobustnessODBenchmark} present the adverse affect of covariate shift on the accuracy of object detectors using ImageNet-C style corruptions \cite{hendrycks2019robustness}.  
%
Besides, Harakeh and Waslander \cite{RegressionUncOD} show that the uncertainty in the localization task increases as the corruption level gets more severe
%
\paragraph{Comparative Summary}
%
In this paper, we thoroughly investigate different ways of computing detection-level uncertainties and aggregating them into image-level. 
%
Unlike the existing literature \cite{RegressionUncOD,VOS} focusing on uncertainty estimation from detection-level perspective, we show that image-level uncertainties provide useful information, which can be used to reject en entire image, e.g. in the presence of strong covariate shift.
%
Different from existing calibration measures for object detection \cite{CalibrationOD,mvcalibrationod}; based on the definition of the task, we investigate calibration from a joint perspective of classification and localization and require the detection score to be aligned with their joint performance.
%
Finally, we target the bad practices in evaluating object detectors such as using small-scale datasets and exploiting test set to validate the model.
%
Accordingly, we define self-aware object detection and provide a framework including (i) large-scale test datasets including not only ID data but also covariate shift and OOD data (around 400K images for each of our settings), (ii) a set of evaluation measures and (iii) a baseline to convert any object detector to a self-aware one.
%
Note that requiring image-level rejection in self-aware object detection also avoid the grouping of the detections as ID or OOD, which impacts the reliability of evaluation in detection-level \cite{VOS}.
}

==> Sections/5.Calibration-old.tex <==
\section{Calibration of Object Detectors}\label{sec:calibration}
%
Calibration, the alignment of accuracy and confidence of a model, has already been extensively studied for the standard classification task\cite{calibration,AdaptiveECE,verifiedunccalibration,rethinkcalibration,FocalLoss_Calibration,calibratepairwise}.
%
%However, very limited attention is paid to study the calibration properties of an object detector.
Differently for object detection, the goal here is to align a detector's performance with the quality of the joint task of classification and localisation (regression).
%
Arguably, it is not obvious how to extend merely classification-based calibration measures such as Expected Calibration Error (ECE)~\cite{} for object detection.
%
A straightforward extension would be to replace the accuracy in such measures by the precision of the detector, which is computed by validating true-positives.
%
However, this perspective does not account for the fact that two object detectors, while have the same precision, might differ in terms of localization quality. %differ between two detectors, say D1 and D2, with equal precision and D1 has a good localisation performance ($\mathrm{IoU} \approx 1$ for TPs) while the IoUs of TPs for D2 slightly exceed $\tau$, i.e. $\tau + \epsilon$ with small $\epsilon$; hence it would not be an ideal measure for object detection.
%

Hence, as one of the main contributions of this work, we consider the calibration of object detectors from a fundamental perspective and define a Localisation-aware Expected Calibration Error (LaECE) which takes into account the joint nature of the task (classification and localisation).
%
We further analyse how calibration measures should be coupled with accuracy in object detection and adapt common calibration methods such as histogram binning, linear regression, and isotonic regression to improve LaECE.
%
%Overall, we take an important step to understand this challenging problem for object detection.
%
% we first propose the calibration error for object detectors which incorporates classification and localisation accuracy.
%
% Then, we investigate the effect of coupling our calibration error with different accuracy measures (AP and LRP) and evaluate the models using typical calibration methods such as: isotropic regression; histogram binning and linear regression.
%
% Furthermore, we also highlt critical defficiencies of the AP metric
%
% \subsection{Object Detection Calibration Error}
%
%
%The data distribution in an object detection set is represented as $c, b, \mathbf{x} \sim \mathbb{P}(C, B, X)$, where $j$ indicates an i.i.d sample.
%
%For a calibrated model we seek to ensure
%
%\begin{align}\label{eq:gen_calibration}
%    \mathbb{P}(C_i = \hat{c}_i, F_{B_i}(B_i) \ge 1 - \hat{p}_i | P = \hat{p}_i) = P \quad \forall P \in [0, 1]
%\end{align}
%
%for a hypothetical object detector which yields  $f_J(\mathbf{x}) = \{p_{C_i, B_i}(c, b)\}^N$ for the random variables $C_i \in \{1, ..., K\}$ and $B_i \in \mathbb{R}^{4}$, here $F_{B_i}$ is the marginal CDF of $p_{C_i, B_i}(c, b)$. 
%
%Following Kuleshov et al.\cite{regressionunc}, we use confidence intervals for localisation, which is in fact a regression task, please see App. \ref{app:subsec_cal_relation} for more details.

\begin{figure}[t]
        \captionsetup[subfigure]{}
        \centering
        %
        \begin{subfigure}[b]{0.14\textwidth}
            \includegraphics[width=\textwidth]{Images/calibration_cls.pdf}
            \caption{Classifier \cite{calibration}}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.17\textwidth}
            \includegraphics[width=\textwidth]{Images/calibration_reg.pdf}
            \caption{Regressor \cite{regressionunc}}
        \end{subfigure}
        %
        \begin{subfigure}[b]{0.155\textwidth}
            \includegraphics[width=\textwidth]{Images/iou_borders.pdf}
            \caption{Detector}
        \end{subfigure}
        %
        %\begin{subfigure}[b]{0.235\textwidth}
        %    \includegraphics[width=\textwidth]{Images/ablation/ablation_atss_OOD_threshold.pdf}
        %    \caption{ATSS (Image-level)}
        %\end{subfigure}
        %
        %\begin{subfigure}[b]{0.235\textwidth}
        %    \includegraphics[width=\textwidth]{Images/ablation/ablation_atss_ID_threshold.pdf}
        %    \caption{ATSS (Detection-level)}
        %\end{subfigure}
        %
        \caption{Illustrations for \textbf{(a)} calibrated classifier, \textbf{(b)} bayesian regressor (Blue dots: ground truths, x: examples and y: target domain) and \textbf{(c)} an object detector. In \textbf{(b)}, we visualize one approach of calibrated regression \cite{regressionunc}, see text for the other. In \textbf{(c)}, we illustrate the boundaries of IoU for different values in image space, e.g., any box obtained from a point within top-left and bottom-right green loci has $\mathrm{IoU} > 0.2$ with the blue box \cite{BBSampling}. The detector is calibrated if its confidence aligns both with its precision as the classification quality and IoU as the localisation quality.
        }
        \label{fig:calibration_def}
\end{figure}

\subsection{Localisation-aware ECE} \label{subsec:mECE}
%
% Here we introduce a core contribution of this work, the Object Detector ECE, termed laECE, which measures the calibration error for object detectors. 
%
%Let $\hat{p}_i$ denotes the detection confidence score corresponding to the $i$-th bounding box. 
Here we obtain Localisation-aware ECE in which the detection confidence score $\hat{p}_i$ accounts for both classification and localisation performance.
%
While $\hat{p}_i$ has been simply obtained only by considering the classification confidence by the earlier detectors \cite{SSD,FasterRCNN,FocalLoss,RFCN}, the recent approach in the literature is to combine localisation and classification confidences in $\hat{p}_i$, which is shown to be effective for improving the accuracy \cite{IoUNet,KLLoss,FCOS,GFL,varifocalnet,GFLv2,aLRPLoss,RSLoss,RankDetNet,paa}.
%
To do so, while the methods exploit different approaches, one common example is to train an additional auxiliary head to regress the localisation quality (e.g., IoU) of the predictions \cite{IoUNet,paa,FCOS,ATSS,KLLoss,maskscoring,yolact-plus}, which can be interpreted as the localisation confidence.
%
Then during inference, the predicted classification confidence is combined with the localisation confidence, e.g., commonly through their product \cite{IoUNet,FCOS,ATSS,maskscoring,yolact-plus}, so that $\hat{p}_i$ now represents the joint confidence.
%
In our derivation, we adopt this recent perspective as it also aligns with the joint nature of the object detection; hence we expect $\hat{p}_i$ to reflect the joint quality of the prediction to enable the subsequent systems to decide properly.

\textbf{An Intuitive Interpretation of the Calibration of Detectors}
%
In order to interpret the calibration of object detectors, we first revisit its subtasks and briefly discuss what a calibrated classifier and a calibrated regressor correspond to.
%
For the former, the widely-adopted definition is that a classifier is calibrated if its confidence matches its accuracy as illustrated in \cref{fig:calibration_def}(a) \cite{calibration,AdaptiveECE,verifiedunccalibration,rethinkcalibration,FocalLoss_Calibration,calibratepairwise}.
%
As for calibrated bayesian regressor, which outputs a distribution instead of a single prediction, there are different approaches for its definition \cite{regressionunc,distributioncalibrationregression,UCE,UCE2}.
%
One notable definition \cite{regressionunc} requires aligning the predicted and empirical cumulative distribution functions (cdf), implying $p\%$ credible interval from the mean of the predictive distribution should include $p\%$ of the ground truths for $p \in [0,1]$ (\cref{fig:calibration_def}(b)).
%
However, extending this definition to object detection is nontrivial due to the increasing complexity of the problem.
%
For example, a detection is represented by a tuple $\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$ with $\hat{b}_i \in \mathbb{R}^{4}$, which is not univariate as in \cite{regressionunc}, and besides, $\hat{p}_i$ accounts for the joint confidence, hence, it is not obvious neither to obtain nor to incorporate the cdf.
%
More importantly, this definition to align the empirical and predicted cdfs does not consider the regression error or accuracy explicitly, and therefore, it is not fit for our purpose.
%
Instead, we follow the alternative definition that aims to directly align the confidence (or uncertainty) with the regression accuracy (or error) \cite{UCE,UCE2}.
%
To illustrate, UCE \cite{UCE} and ENCE \cite{UCE2} require a calibrated regressor to match the predicted variance with the expected error, e.g., the mean squared error. 
%
In our case, we exploit IoU, the de-facto localisation quality for object detection and illustrate how different IoU boundaries look like in the image-space using the expressions derived by Oksuz et al. \cite{BBSampling} in \cref{fig:calibration_def}(c).
%
In particular, any prediction box can be mapped onto the blue box in \cref{fig:calibration_def}(c) since IoU is translation- and scale-invariant \cite{BBSampling}, hence the locus for different IoUs provide an intuition on where the ground truth box can reside depending on the predicted confidence $\hat{p}_i$.
%
Following from those, we say that an object detector, $f(X) = \{\hat{c}_i, \hat{b}_i, \hat{p}_i\}^N$ with $\hat{c}_i \sim C_i$, $\hat{b}_i \sim B_i$ and $\hat{p}_i \sim P_i$, is calibrated if $P_i$ matches the product of (i) the probability that $\hat{C}_i$ is accurate and (ii) expected localisation quality of $B_i$ for $\forall \hat{p}_i \in [0, 1]$, which is similar to how common detectors obtain $\hat{p}_i$ as aforementioned.
%
Formally, a calibrated object detector ensures $\forall \hat{p}_i \in [0, 1]$,
%
% $\hat{B}_i \in \mathcal{B}(\hat{p}_i)$ where $\mathcal{B}(\hat{p}_i)$ is the set of boxes that fall in a region around some IoU, which can be illustrated as the vicinity of a certain locus in \cref{fig:calibration_def}(c).
%
\par\nobreak
{\small
\begin{align}\label{eq:gen_calibration_}
    \mathbb{P}(C_i = \hat{c}_i| P_{i} = \hat{p}_i) \mathbb{E}_{B_i}( \mathrm{IoU}(B_i, B_{\psi(i)}) | P_{i} = \hat{p}_i) = \hat{p}_i,
\end{align}
}%

\par\nobreak
{\small
\begin{align}\label{eq:gen_calibration_}
    \mathbb{P}(C_i = \hat{c}_i| \hat{p}_i) \mathbb{E}_{B_{i}}(\mathrm{IoU}(\hat{b}_i , b_{\psi(i)} ) \in \mathcal{R}(\hat{p}_i)| \hat{p}_i) = \hat{p}_i,
\end{align}
}

%
%and $\hat{p}_{i}$ can be expressed as, 
%
%\begin{align}\label{eq:score}
%    \hat{p}_{i} = \hat{p}_{i}^{cls} \times \hat{p}_{i}^{loc},
%\end{align}
%
%where $\hat{p}_{i}^{cls}$ and $\hat{p}_{i}^{loc}$ are the confidence scores for classification and localisation respectively. 
%
where $B_{\psi(i)}$ is the ground truth box that $i$th prediction matches with.
%
Note that Eq. \eqref{eq:gen_calibration_} consists of two terms:
%
$\mathbb{P}(C_i = \hat{c}_i | P_{i}=\hat{p}_i)$ is the ratio of the number of correctly-classified detections ($\mathrm{N_{TP}}$) and the total number of detections ($\mathrm{N_{TP}} + \mathrm{N_{FP}}$), which is simply the precision representing the classification quality; and
%
$\mathbb{E}_{P_{i}}( \mathrm{IoU}(B_i, B_{\psi(i)})$ represents the localisation quality in terms of IoU and is defined for TP detections.
%
Note that when there is no TP, then the precision is $0$ and $\hat{p}_i$ should naturally be $0$.
%
As intended, Eq. \eqref{eq:gen_calibration_} requires a higher $\hat{p}_i$ as precision or localisation quality of the detector increases, and besides, it only relies on the conventional output of a detector $\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$; thereby allowing us to compute the calibration error for any object detector.

\paragraph{Puneet}
Let $\hat{p}_i$ be the output confidence score of a detector corresponding to the predicted tuple $\{\hat{b}_i, \hat{c}_i\}$. Then, the detector is calibrated over a data distribution $\mathcal{D}$ if over all the $(b_i, c_i)$ pairs in $\mathcal{D}$ the probability that $\hat{c}_i = c_i$ \textit{and} $\mathrm{IoU}(\hat{b}_i, b_i) \in  \mathcal{R} (\hat{p}_i)$ is $\hat{p}_i$, where $\mathcal{R} (\hat{p}_i)$ is a small non-zero interval around $\hat{p}_i$. More formally, %assuming $\mathbb{P}$ to be the joint distribution betweeen $\{\hat{p}_i, \hat{b}_i, \hat{c}_i\}$
{\small
\begin{align}\label{eq:gen_calibration_}
    \mathbb{P}(\hat{c}_i = c_i \; \& \; \mathrm{IoU}(\hat{b}_i, b_i) \in  \mathcal{R} (\hat{p}_i) | \; \hat{p}_i) = \hat{p}_i, \forall \hat{p}_i \in [0,1]
\end{align}
}%
For simplicity, we assume the two events to be independent\footnote{Note, though we assume independence assumption for mathematical simplicity, the model is already trained in a way to produce detections that assigns correct label to a set of tight bounding-boxes around the object of interest.}

{\small
\begin{align}\label{eq:gen_calibration_}
    \mathbb{P}(\hat{c}_i = c_i | \; \hat{p}_i) \mathbb{P}(\mathrm{IoU}(\hat{b}_i, b_i) \in  \mathcal{R} (\hat{p}_i) | \; \hat{p}_i) = \hat{p}_i, \forall \hat{p}_i \in [0,1]
\end{align}
}%

\textbf{LaECE and its Practical Usage} 
%
We define LaECE as the expected calibration error of a detector based on Eq. \eqref{eq:gen_calibration_}.
%
While doing so, we compute the average calibration error over classes following performance measures in object detection \cite{COCO,LVIS,Objects365,OpenImages, LRPPAMI} to prevent more frequent classes to dominate the calibration error; and discretize the confidence score space into $J$ equally-spaced bins by splitting the detections into these bins for each class ($J^{c}=25$ for class $c$) similar to \cite{calibration,verifiedunccalibration}.
%
Consequently, we define the calibration error for a class $c$, denoted by $\mathrm{LaECE}^c$, as the weighted average of the differences of the confidence score from the product of precision ($\mathrm{precision}^{c}(j)$) and average IoU of TPs ($\bar{\mathrm{IoU}}^{c}(j)$)
%
\par\nobreak
{\small
\begin{align}
\label{eq:odcalibrationfinal1}
   \mathrm{LaECE}^c 
   & = \sum_{j=1}^{J^{c}} \frac{|\hat{\mathcal{D}}^{c}_j|}{|\hat{\mathcal{D}}^{c}|} \left\lvert \bar{p}^{c}_{j} - \mathrm{precision}^{c}(j) \times \bar{\mathrm{IoU}}^{c}(j)  \right\rvert,
\end{align}}
%
where $\hat{\mathcal{D}}^{c}$ denotes the set of all detections, $\hat{\mathcal{D}}_j^{c}	\subseteq \hat{\mathcal{D}}^{c}$ is the set of detections in bin $j$ and $\bar{p}_{j}^{c}$ is the average of the detection confidence scores in bin $j$ for class $c$. 
%
Then, $\mathrm{LaECE}$ of an object detector is the average over $\mathrm{LaECE}^c$ for $c \in \{1, ..., K\}$.
%
Thus, we have presented a tractable approach to compute the calibration error of object detectors accounting for both classification \emph{and} localisation.

\subsection{The Curse of Top-k Survival} \label{subsec:relation}
% Outcome: don't use top-k

% Why? in situations with few detections/objects top-k will implicitly incoprorate these noisy detections into the evaluation. This can be seen in Fig 4a, where filling the remaining top-k detections with zero conf dummies, leads to an improvement in laECE, without actually seeing a corresponding change in AP.
% %
% This high sensitivy to the remaining top-k detections, is unwanted and potentially leads to misinterpreted results Fig 4a.

% What do we want to use instead? Here we actually want to select the most appropriate detections based on their uncertainties.

% LRP is requires a balanced set of errors for precision, recall and localisation.
%
A critical stage in the detection pipeline is to obtain the final detections from raw detections, termed postprocessing generally including background removal, NMS and finally top-$k$ survival (\cref{sec:relatedwork}).
%
Top-$k$ survival selects $k$ detections with the highest confidence, where $k$ is typically significantly larger than the number of objects in an image, e.g., $k=100$ for COCO with an average of 7.3 objects per image on its val set.
%
Evidently, the final detections can contain numerous low-scoring noisy detections after top-$k$ survival; ATSS has for example 86.4 detections per image, far more than the average number of objects in an image on the COCO val set. 

However these noisy detections induced by top-$k$ survival might not have an affect on a performance measure while it has an affect on LaECE.
%
%these noisy detections may (or may not) have an impact on the score.
%
We demonstrate this by a synthetic experiment in \cref{fig:calibration}(a):
%Here, in order to explore LaECE and match it with a proper accuracy measure, we investigate the effect of such low-scoring detections with a simple approach:
%
Specifically, if the number of final detections is less than $k$ for an image, then we insert ``dummy'' detections into the remaining space.
%
These dummy detections randomly predict a class $\hat{c}_i$ with $\hat{p}_i = 0$ and do not match with an object owing to covering an area of 1 pixel, hence they are ``perfectly calibrated''.
%
Inserting these dummy detections artificially reduces LaECE, which decreases as $k$ increases (solid line in \cref{fig:calibration}(a)).
%
This is because the weight of the first bin ($|\hat{\mathcal{D}}^{c}_j|/|\hat{\mathcal{D}}^{c}|$ for $j=1$ in Eq. \eqref{eq:odcalibrationfinal1}) increases relative to other bins while its error ($\left\lvert \bar{p}^{c}_{j} - \mathrm{precision}^{c}(j) \times \bar{\mathrm{IoU}}^{c}(j)  \right\rvert$) decreases since precision and confidence are both $0$ for such detections.
%
On the other hand, AP is completely unaffected when adding these dummy detections; giving the false impression that the calibration performance of the detector has increased.
%
We also prove in App. \ref{app:calibration} that AP is not affected by such dummy detections by definition and promotes low scoring noisy detections.
%
For this reason, \textit{we do not advocate top-$k$ survival, instead, we motivate the need to select a properly-thresholded set of detections with a good balance of precision, recall and localisation errors to consistently evaluate the calibration performance of object detectors}\footnote{Using properly-thresholded detections is in fact similar to the Panoptic Segmentation, which is a closely-related task to object detection \cite{PanopticSegmentation,PanopticFPN}}.
%

%Hence, we require a properly-thresholded set of detections with a good balance of precision, recall and localisation errors while using LaECE.
%
%Furthermore, as can be seen in Fig. \ref{fig:calibration}(a), we also note that AP is completely unaffected when adding these dummy detections.
%
We impose that by using LRP Error \cite{LRPPAMI} (\cref{sec:relatedwork}), which is sensitive to the dummy (and noisy) detections (dotted line in Fig. \ref{fig:calibration}(a) and \ref{fig:calibration}(b)) due to the inclusion of FPs in Eq. \eqref{eq:LRPdefcompact}.
%
While using LRP Error and LaECE, both of which consider the localisation quality of a TP precisely, we validate the TPs from an IoU of $\tau=0.10$, for which LaECE is not sensitive between $0.00$ and $0.50$ as shown in App. \ref{app:calibration}.
%
This also aligns with how common analysis tools of object detectors decompose classification and localisation errors \cite{Analyzer,TIDE}; thereby providing a proper joint evaluation.
%
% This is unsurprising as LRP Error requires properly thresholded detections, thereby implicitly addressing the issues associated with top-$k$ survival and AP.
%
In \cref{fig:calibration}(b), we present the effect of the detection score threshold on LRP Error, where the lowest error is obtained around 0.30 for ATSS and 0.70 for F R-CNN, leading to an average of 6 detections/image for both detectors, far closer to the average number of objects compared to using $k=100$.
%
Finally, for thresholding the detections in SAODets, we use LRP-optimal thresholding \cite{LRPPAMI}, which is the threshold achieving the minimum LRP Error for each class on the val set.

%
%
% %While top-k survival (and AP) does not prevent this trivial way to improve laECE (see AP is constant over $k$ in Fig. \ref{fig:calibration}(a)); LRP Error penalizes the dummy detections significantly owing to increasing number of positives (Eq. \eqref{eq:LRPdefcompact}), thereby avoiding an improvement in laECE simply by including dummy detections.
% %
%% On the other hand, LRP Error requires properly thresholded detections, that is, the detections are to have a good balance of precision, recall and localisation errors\footnote{This way of evaluation is also being used by Panoptic Segmentation exploiting Panoptic Quality \cite{PanopticSegmentation,PanopticFPN}.}.
% %
% %\paragraph{Detection-level thresholding.} 
% Fig. \ref{fig:calibration}(b) presents more insight on this: LRP Error reaches minimum with around 6 det/img for both detectors, AP is maximized when there is no threshold (none) and average detections per image (det/img) is the largest, e.g., it is $86.4$ for ATSS significantly higher than $7.3$ objects/image existing in COCO val set.
% %
% %Besides, this large set of detections (e.g., $86.4$ for ATSS) promoted by AP is barely useful in practice.
% %
% As a result, we couple laECE with LRP Error to prevent aforementioned trivial way of improving calibration performance and to encourage the object detectors to yield rather useful detections by discarding low-scoring noisy ones.
%
%In our experiments, we use class-wise LRP-Optimal thresholds \cite{LRPPAMI} obtained on val sets for thresholding purpose. 
%that correspond to the minimum LRP Error on val set and capture the differences across detectors (e.g., at $0.70$; while Faster R-CNN achieves a low LRP Error, ATSS is almost useless with a very high LRP Error).
%Armed with a method to evaluate the calibration error of object detectors, we now explore its link between itself and accuracy.
%
%One would expect that artificially increasing the number of true negatives in a set of detections should result in an improvement in accuracy and a change in laECE.
%
%Here we explore this hypothesis by artificially introducing more true negatives, where we fill the remaining space in top-$k$ survival with `dummy' detections.
%
%These dummy detections set $\hat{p}_i = 0$ with a randomly predicted $\hat{c}_i$ and do not match with an object owing to covering an area of 1 pixel, hence they are ``perfectly calibrated'' true negatives and reside in the first bin.
%
%Doing so, we would expect to see the laECE improve \emph{and} a change in the accuracy.
%
%In fact, Fig. \ref{fig:calibration}(a) shows the contrary for AP: Simply by filling the remaining space of top-100 survival used by AP with `dummy' detections superficially decrease laECE, whilst keeping the AP constant.
%
%Besides, increasing $k$ decreases laECE down to $\sim 0$.
%
%Clearly AP does not capture this trivial way to improve laECE by staying the same for any $k$ (dashed lines in Fig. \ref{fig:calibration}(a)); LRP Error (dotted lines) penalizes the dummy detections significantly (F R-CNN degrades from $86.5$ to $96.8$ with up to 100 dummy detections), preventing this undesired effect.
%
%Unlike AP relying on top-k survival, LRP Error instead selects the detections if they are greater than a pre-determined threshold, resulting in them having a good balance of precision, recall and localisation error\footnote{This way of evaluation is also being used by Panoptic Segmentation exploiting Panoptic Quality \cite{PanopticSegmentation,PanopticFPN}. 
%
%Also, depending on the use-case, the contribution of each error type on LRP Error can be set differently \cite{LRPPAMI}}.
%
%\paragraph{Detection-level thresholding.} 
%Fig. \ref{fig:calibration}(b) presents more insight into this effect: While AP is maximized when there is no threshold (none) and the average detections per image (det/img) is the largest, LRP Error reaches a minimum closer to $7.3$ obj/img of COCO val set, that is around 6 det/img for both detectors.
%
%Besides, this large set of detections (e.g., $86.4$ for ATSS) promoted by AP is barely useful in practice.
%
%Consequently, for thresholding purpose, rather than using AP we use class-wise LRP-optimal thresholds that correspond to the minimum LRP Error on val set and capture the differences across detectors (e.g., at $0.70$; while Faster R-CNN achieves a low LRP Error, ATSS is almost useless with a very high LRP Error).
\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.07em}
    \def\r{\hspace*{1.0ex}}
    \small
    \caption{How different calibration methods LaECE and LRP. \xmark: No calibration, HB: Histogram binning, IR: Isotonic Regresssion, LR: Linear Regression. ATSS, combining localisation and classification confidences through multiplication as in our LaECE (Eq. \eqref{eq:odcalibrationfinal1}), performs the best on both datasets before/after calibration. Aligned with \cite{FocalLoss_Calibration}, uncalibrated F R-CNN using cross-entropy loss performs the worst.}
    \label{tab:calibratingod}
    \scalebox{0.85}{
    \begin{tabular}{c@{\r}|@{\r}c@{\r}c@{\r}c@{\r}c@{\r}|@{\r}c@{\r}c@{\r}c@{\r}c@{\r}|@{\r}c@{\r}c@{\r}c@{\r}c@{\r}|@{\r}c@{\r}c@{\r}c@{\r}c@{\r}|@{\r}c@{\r}c@{\r}c@{\r}c@{\r}|@{\r}c@{\r}c@{\r}c@{\r}c@{\r}}
    \toprule
    \midrule
    Dataset &\multicolumn{16}{c@{\r}|@{\r}}{SAOD-Gen}&\multicolumn{8}{c}{SAOD-AV} \\
    \midrule
    Detector &\multicolumn{4}{c@{\r}|@{\r}}{F R-CNN}&\multicolumn{4}{c@{\r}|@{\r}}{RS R-CNN}&\multicolumn{4}{c@{\r}|@{\r}}{ATSS}&\multicolumn{4}{c@{\r}|@{\r}}{D-DETR}&\multicolumn{4}{c@{\r}|@{\r}}{F R-CNN}&\multicolumn{4}{c}{ATSS} \\
    Calibrator&\xmark&LR&HB&IR&\xmark&LR&HB&IR&\xmark&LR&HB&IR&\xmark&LR&HB&IR&\xmark&LR&HB&IR&\xmark&LR&HB&IR \\
    \midrule
    LaECE&$43.3$&$17.7$&$18.6$&$\mathbf{16.9}$&$32.0$&$17.4$&$19.6$&$\mathbf{17.2}$&$\mathbf{15.7}$&$16.8$&$18.7$&$16.7$&$15.9$&$\mathbf{15.7}$&$17.7$&$15.9$&$26.5$&$\mathbf{9.8}$&$10.2$&$10.2$&$16.8$&$\mathbf{9.0}$&$9.7$&$9.7$ \\
    
    LRP&$74.7$&$74.7$&$74.7$&$74.7$&$73.6$&$73.6$&$73.6$&$73.6$&$74.0$&$74.0$&$74.1$&$74.0$&$71.9$&$71.9$&$71.9$&$71.9$&$73.5$&$73.5$&$73.5$&$73.5$&$70.6$&$70.6$&$70.6$&$70.6$  \\
    \midrule
    \bottomrule
    \end{tabular}
    }
\end{table*}

\begin{figure}[t]
        \captionsetup[subfigure]{}
        \centering
        \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\textwidth]{Images/reliabilitydiagrams/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_identity_thresholding_reliabilitydiagram.pdf}
        \caption{Uncalibrated}
        \end{subfigure}
        \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\textwidth]{Images/reliabilitydiagrams/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_linear_regression_thresholding_reliabilitydiagram.pdf}
        \caption{Calibrated by LR}
        \end{subfigure}
        \caption{Reliability diagrams of F R-CNN on $\mathcal{D}_{\mathrm{ID}}$ of SAOD-Gen before/after calibration. We use Precision$\times \mathrm{\bar{IoU}}$ based on Eq. \eqref{eq:odcalibrationfinal1}. Calibration by LR decreases overconfidence of F-RCNN.}
        \label{fig:frcnnreliabilityhist}
\end{figure}

\subsection{Calibration Methods and Reliability Diagrams} \label{subsec:calibrationmethods}
%
Now, we adapt common calibration methods to improve LaECE.
%
To do so, for each class, we train a calibrator $\zeta^c:[0,1] \rightarrow [0,1]$ using input-target pairs ($\{x^{cal}_i, y^{cal}_i\}$) derived from the detections ($\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$) on the val set.  
%
Since we want to map the confidence scores, we simply set $x^{cal}_i=\hat{p}_i$ in the training set of class $\hat{c}_i$.
%
As for its target $y^{cal}_i$, we show in App. \ref{app:calibration} that LaECE in $j$th bin (Eq. \eqref{eq:odcalibrationfinal1}) reduces to
%
{\small
\begin{align}
\label{eq:finalECEoptimise_main}
  &\left\lvert \sum_{\hat{b}_i \in \hat{\mathcal{D}}_j^c, \psi(i) > 0} \left( \hat{p}_{i} - \mathrm{IoU}(\hat{b}_i, b_{\psi(i)}) \right) + \sum_{\hat{b}_i \in \hat{\mathcal{D}}_j^c, \psi(i) \leq 0} \hat{p}_{i}  \right\rvert.
\end{align}}%
%
Eq. \eqref{eq:finalECEoptimise_main} and LaECE is minimized if (i) $\hat{p}_{i}=\mathrm{IoU}(\hat{b}_i, b_{\psi(i)})$ for TPs ($\psi(i) > 0$), hence we set $y^{cal}_i=\mathrm{IoU}(\hat{b}_i, b_{\psi(i)})$ for TPs; (ii) $\hat{p}_{i}=0$ for FPs ($\psi(i) \leq 0$), hence $y^{cal}_i=0$ for FPs.
%

%As we elaborate more on in Supp.Mat., this way of constructing the training pairs aligns with the proposed laECE.
%In situations, where $x^{cal}_i = \hat{y}^{cal}_i$, the corresponding laECE becomes zero.

Specifically, we train linear regression (LR); histogram binning (HB); and isotonic regression (IR) models with such pairs.
%
%We report the results on our ID test sets in Table \ref{tab:calibratingod} with an example reliability diagram in Fig. \ref{fig:frcnnreliabilityhist} (see App. \ref{app:calibration_analyses} for more examples).
\cref{tab:calibratingod} shows that these calibration methods improve LaECE for five out of six cases, and in the case where they perform worse (ATSS on SAOD-Gen), the calibration performance is already good. 
%
Overall we find IR and LR perform better than HB and we employ LR for SAODets since LR performs the best on three detectors. 

%
We also exploit reliability diagrams to provide insight on the calibration of a detector (\cref{fig:frcnnreliabilityhist}).
%
To obtain a reliability diagram, we first obtain the performance, measured by the product of precision and IoU (Eq. \eqref{eq:odcalibrationfinal1}), for each class over bins and then average the performance over the classes by ignoring the empty bins. 
%
Note that if a detector is perfectly calibrated with $\mathrm{LaECE}=0$, then all the histograms will lie along the diagonal in the reliability diagram since $\mathrm{laECE}^c=0$ for $c \in \{1, ..., K\}$.
%
Similar to classification, if the performance tends to be lower than the diagonal, then the detector is said to be over-confident as in Fig. \ref{fig:frcnnreliabilityhist}(a), and vice versa for an under-confident detector. 

%Supp.Mat. presents that the models trained under this procedure with HB and IR yield $0$ laECE on the validation set, implying the accuracy of our dataset construction scheme.
%
%Table \ref{tab:calibratingod} presents the results and we also include reliability diagram superimposed with the distribution of the samples pertaining to F R-CNN in Fig. \ref{fig:frcnnreliabilityhist}:
%
% Table \ref{tab:calibratingod} shows that these calibration methods yield improved laECE for five out of six cases, and in the case where they perform worse (ATSS on Gen-OD), the calibration performance is already good. 
%
%In terms of calibration approaches, overall we find IR and LR perform better than HB; consequently we employ LR for the rest of the paper.
%
% Especially, F R-CNN, which is over-confident (Fig. \ref{fig:frcnnreliabilityhist}), improves notably without any effect on its accuracy.
% %
% The exception is ATSS (Gen-OD), where $\hat{p}_i$ is the product of the classification confidence scores and the centerness scores predicted by an additional head, which can be considered as a proxy localisation quality.
% %
% This consequently
%
% which is inherently better-calibrated since the detection scores ($\hat{p}_i$) are obtained following the definition of ECE (Eq. \eqref{eq:odcalibrationfinal}).
% %
% Particularly, for ATSS, $\hat{p}_i$ is the product of the classification confidence scores and the centerness scores predicted by an additional head, which can be considered as a proxy localisation quality.
%
% naturally predicts very good confidence estimates, and applying temperature calibration simply makes us overfit to the confidence.
%
%Overall IR and LR perform better than HB and we employ LR for the rest of the paper considering that LR performs the best on three detectors.
%
%(i) Different from calibrating classifiers, calibration methods can affect accuracy when they affect the rankings of the detections. 
%
%As an exception; fitting a line, LR does not affect the ranking of the detections, thereby guaranteed to preserve accuracy (Table \ref{tab:calibratingod}). 
%
%(ii) Calibration methods improves laECE especially for top-100 survival since it is dominated by the first bin with very low confidence scores (Table \ref{tab:calibratingod}, Fig. \ref{fig:frcnnreliabilityhist}(a) and (b)). 
%
%(iii) Calibrating for thresholded detections is more challenging. While F R-CNN and RS R-CNN improve, we haven't observed notable improvement for ATSS and D-DETR (Table \ref{tab:calibratingod}, Fig. \ref{fig:frcnnreliabilityhist}(c) and (d)). 
%
%Considering that IR, in general, performs better, we employ IR for the rest of the paper.
%


\blockcomment{
%
\paragraph{Issues with AP}
%
Moreover, this experiment highlights critical issues with the AP metric.
%
Specifically, the number of there eroneous dummy detections does not affect the AP.
%
In more detail, the failures of AP can broadly described as the folowing:
\begin{itemize}
    \item Localisation quality of the prediction is only taken into account in a `step-wise' manner.
    %
    I.e. only once the IoU meets a certain threshold is it counted towards AP, and even then, the quality of IoU has no effect on the final value of AP.
    %
    \item Given that the AP is calculated as the area under the PR curve, there are potentially infinite detector characteristics which lead to the same value of AP.
    %
    This forces researchers to investigate further metrics such FN, TP and average recal.
\end{itemize}
%
For a more comprehensive critique, we direct the readers towards~\cite{LRPPAMI}.
%
Conseqently, we utlise the LRP Error (Eq. \eqref{eq:LRPdefcompact})\footnote{Note that this way of performance evaluation has already been used by Panoptic Segmentation benchmark exploiting Panoptic Quality \cite{PanopticSegmentation,PanopticFPN} as the performance measure}, which, as be can seen \ref{tab:dummydet}, captures the change in predictions once dummy detections are added.
%
However, this introduces the additional problem of what is the appropriate value for thresholding the detections.
%, which we explore next.
}
%
%
\blockcomment{
\begin{table}
    \centering
    \setlength{\tabcolsep}{0.1em}
    \caption{In order to promote the detection output to be aligned with the practical usage and prevent superficial improvement of calibration performance, we require the detections to be thresholded properly by adopting LRP. COCO minival has 7.3 objects/image.}
    \label{tab:threshold}
    \begin{tabular}{|c|c|c|c|c|c|c|} \hline
         Detector&Threshold&det/img.&$\mathrm{laECE}$&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{LRP}$ \\ \hline
    \multirow{5}{*}{F R-CNN}&None&$33.9$&$15.11$&$39.9$&$67.5$&$86.5$\\
    &0.30&$11.2$&$27.48$&$38.0$&$67.5$&$67.6$\\
    &0.50&$7.4$&$27.60$&$36.1$&$67.6$&$62.1$\\
    &0.70&$5.2$&$24.49$&$33.2$&$68.4$&$61.5$\\ \cline{2-7}
    &LRP-opt.&$6.1$&$26.08$&$34.6$&$67.9$&$61.1$\\\hline
    \multirow{5}{*}{ATSS}&None&$86.4$&$7.69$&$42.8$&$65.7$&$95.1$\\
    &0.30&$5.2$&$20.18$&$35.3$&$66.7$&$60.5$\\
    &0.50&$2.0$&$26.64$&$19.7$&$80.7$&$78.4$\\
    &0.70&$0.3$&$12.32$&$3.9$&$96.5$&$96.3$\\ \cline{2-7}
    &LRP-opt.&$6.0$&$18.25$&$36.7$&$66.2$&$60.2$\\ \hline
    \end{tabular}
\end{table}
    \begin{table}
        \centering
        \small
        \setlength{\tabcolsep}{0.03em}
        \caption{In order to promote the detection output to be aligned with the practical usage and prevent superficial improvement of calibration performance, we require the detections to be thresholded properly by adopting LRP. COCO minival results with 7.3 objects per image.}
        \label{tab:threshold}
        \begin{tabular}{|c|c|c|c|c|c|c|} \hline
             Detector&Threshold&det/img.&$\mathrm{laECE}$&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{LRP}_{0.1}$ \\ \hline
        \multirow{5}{*}{Faster R-CNN}&None&$33.9$&$15.11$&$39.9$&$67.5$&$86.5$\\
        &0.30&$11.2$&$27.48$&$38.0$&$67.5$&$67.6$\\
        &0.50&$7.4$&$27.60$&$36.1$&$67.6$&$62.1$\\
        &0.70&$5.2$&$24.49$&$33.2$&$68.4$&$61.5$\\ \cline{2-7}
        &LRP-opt.&$6.1$&$26.08$&$34.6$&$67.9$&$61.1$\\\hline
        \multirow{5}{*}{ATSS}&None&$86.4$&$7.69$&$42.8$&$65.7$&$95.1$\\
        &0.30&$5.2$&$20.18$&$35.3$&$66.7$&$60.5$\\
        &0.50&$2.0$&$26.64$&$19.7$&$80.7$&$78.4$\\
        &0.70&$0.3$&$12.32$&$3.9$&$96.5$&$96.3$\\ \cline{2-7}
        &LRP-opt.&$6.0$&$18.25$&$36.7$&$66.2$&$60.2$\\ \hline
        \multirow{5}{*}{RS R-CNN}&None&$100$&$41.90$&$42.0$&$66.0$&$96.0$\\
        &0.30&$97.9$&$20.18$&$42.0$&$66.0$&$95.9$\\
        &0.50&$31.2$&$44.52$&$41.8$&$66.0$&$85.5$\\
        &0.70&$4.3$&$9.62$&$32.7$&$68.3$&$62.1$\\ \cline{2-7}
        &LRP-opt.&$5.8$&$16.71$&$36.3$&$66.4$&$59.7$\\ \hline
        \multirow{5}{*}{D-DETR}&None&$100$&$7.77$&$44.3$&$64.2$&$95.8$\\
        &0.30&$8.1$&$11.94$&$40.1$&$64.2$&$58.5$\\
        &0.50&$3.6$&$11.62$&$30.9$&$69.4$&$63.9$\\
        &0.70&$1.8$&$9.51$&$18.8$&$81.5$&$79.2$\\ \cline{2-7}
        &LRP-opt.&$6.3$&$11.22$&$38.2$&$64.5$&$57.2$\\ \hline
        \end{tabular}
    \end{table}


\begin{figure}[ht]
        \captionsetup[subfigure]{}
        \centering
        \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{Images/thr000_174482.png}
        \caption{top-100 survival}
        \end{subfigure}
        \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{Images/thr030_174482.png}
        \caption{thresholding}
        \end{subfigure}
        \caption{The detections obtained by top-100 survival vs. thresholding using ATSS detector. Evaluating the thresholded detections aligns with the practical usage better.}
        \label{fig:threshold_example}
\end{figure}
}
%
%
%We finally note that while we prefer equal contributions of each error type in LRP Error (Eq. \eqref{eq:LRPdefcompact}); depending on the use-case, they can be set differently \cite{LRPPAMI}.
%
% Note that this way of performance evaluation has already been used by Panoptic Segmentation benchmark exploiting Panoptic Quality \cite{PanopticSegmentation,PanopticFPN} as the performance measure

%this approach yields the best LRP Error as expected on val set (Table \ref{tab:threshold}); this problem, we refer as \textit{detection-level thresholding}, is more challenging since different detectors can have significantly different score distributions (e.g. while Faster R-CNN achieves low LRP Error at $0.70$, that of ATSS is close to $100 \%$, implying ATSS is almost useless at $0.70$) and the domain shift can potentially have adverse affects. 
%
%Accordingly, we use class-specific LRP-optimal thresholds \cite{LRPPAMI} to threshold ``noisy'' detections in an image. 
%
%Table \ref{tab:threshold} suggests that LRP-optimal thresholds close the gap between detections/image for F R-CNN and ATSS making them closer to $7.3$ as the average number of objects in the validation set\footnote{While we prefer to penalize false positives and false negatives equally in LRP Error; depending on the application, the weights of different error types can be set differently.}.
%

%
% Also, as we will see in Section \ref{sec:evaluation}, LRP-optimal thresholds provide a reasonable detection-level thresholds in the presence of domain shift for Gen-OD and AV-OD.
%
% In order to be aligned with the practical usage of object detectors, we use ``all final detections'' of an object detectors. Note that this is different from (i) xxx et al. using raw detections and (ii) \cite{RegressionUncOD} splitting the detections into four as true positives, duplicates, false positives and localisation errors following Hoiem et al. \cite{Analyzer} and discarding the duplicates in the analysis. We split the detections as true positives or false positives similar to performance measures; but differently, in order to decouple classification and localisation errors more properly, we set true positive validation threshold as $\tau=0.10$ following the recent analysis tools \cite{Analyzer,TIDE}.
%

\blockcomment{
\begin{figure}[ht]
        \captionsetup[subfigure]{}
        \centering
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_identity_thresholding_reliabilitydiagram.pdf}
        \caption{Gen-OD \& uncalibrated}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_linear_regression_thresholding_reliabilitydiagram.pdf}
        \caption{Gen-OD \& calibrated}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms/faster_rcnn_r50_fpn_straug_3x_robustodavod_severity_0_identity_thresholding_reliabilitydiagram.pdf}
        \caption{AV-OD \& uncalibrated}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms/faster_rcnn_r50_fpn_straug_3x_robustodavod_severity_0_linear_regression_thresholding_reliabilitydiagram.pdf}
        \caption{AV-OD \& calibrated}
        \end{subfigure}
        \caption{Reliability diagrams of F R-CNN on Gen-OD and AV-OD test sets comparing the performance in terms of the product of precision and mean of IoUs as defined based on Eq. \eqref{eq:odcalibrationfinal}. Linear regression is used in the figures, improving laECE of F R-CNN on both datasets.}
        \label{fig:frcnnreliabilityhist}
\end{figure}

\begin{figure*}[ht]
        \captionsetup[subfigure]{}
        \centering
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_identity_ap_style_reliabilitydiagram.pdf}
        \caption{uncalibrated \& top-k survival}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_ap_style_reliabilitydiagram.pdf}
        \caption{calibrated \& top-k survival}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_identity_thresholding_reliabilitydiagram.pdf}
        \caption{uncalibrated \& thresholding}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_thresholding_reliabilitydiagram.pdf}
        \caption{uncalibrated \& thresholding}
        \end{subfigure}
        \caption{Reliability diagrams of F R-CNN on Gen-OD ID test set comparing the performance in terms of the product of precision and mean of IoUs as defined in Eq. \eqref{eq:odcalibrationfinal}. laECE is dominated by the detections with lower scores before and after calibration (see (a) and (b)). Thresholding only keeps relatively more useful detections, hence not prevents the error to be dominated by low-confidence detections. Isotonic regression improves calibration performance of F R-CNN both for top-k survival and for thresholding.}
        \label{fig:frcnnreliabilityhist}
\end{figure*}

\begin{figure*}[ht]
        \captionsetup[subfigure]{}
        \centering
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_coco_severity_0_identity_ap_style_reliabilitydiagram.pdf}
        \caption{F R-CNN on val (no cal. \& top-k)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_coco_severity_0_isotonic_regression_ap_style_reliabilitydiagram.pdf}
        \caption{F R-CNN on val (cal. \& top-k)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_coco_severity_0_identity_thresholding_reliabilitydiagram.pdf}
        \caption{F R-CNN on val (no cal. \& thr.)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_coco_severity_0_isotonic_regression_thresholding_reliabilitydiagram.pdf}
        \caption{F R-CNN on val (no cal. \& thr.)}
        \end{subfigure}

        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_identity_ap_style_reliabilitydiagram.pdf}
        \caption{F R-CNN on test (no cal. \& top-k)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_ap_style_reliabilitydiagram.pdf}
        \caption{F R-CNN on test (cal. \& top-k)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_identity_thresholding_reliabilitydiagram.pdf}
        \caption{F R-CNN on test (no cal. \& thr.)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_thresholding_reliabilitydiagram.pdf}
        \caption{F R-CNN on test (no cal. \& thr.)}
        \end{subfigure}

        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_identity_ap_style_reliabilitydiagram.pdf}
        \caption{ATSS on test (no cal. \& top-k)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_ap_style_reliabilitydiagram.pdf}
        \caption{ATSS on test (cal. \& top-k)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_identity_thresholding_reliabilitydiagram.pdf}
        \caption{ATSS on test (no cal. \& thr.)}
        \end{subfigure}
        \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_thresholding_reliabilitydiagram.pdf}
        \caption{ATSS on test (no cal. \& thr.)}
        \end{subfigure}
        \caption{Reliability diagrams of F R-CNN (on COCO minival and Robust OD test) and ATSS (on Robust OD test) comparing the performance in terms of the product of precision and mean of IoUs as defined in Eq. \eqref{eq:odcalibrationfinal}. cal. implies that isotonic regression is used to calibrate the detection output. IR helps to decrease laECE for F R-CNN on both top-k survival and thresholded (thr.) detections and ATSS on top-k survival, but not for ATSS on thr. detections, leaving the calibration as an open problem.}
        \label{fig:frcnnreliabilityhist}
\end{figure*}
}
%
\blockcomment{
\begin{table}
    \centering
    \setlength{\tabcolsep}{0.25em}
    \small
    \caption{Effect of calibration methods. \xmark: No calibration, HB: Histogram binning, IR: Isotonic Regresssion, LR: Linear Regression. The models are trained on validation set and the results are presented on Gen-OD test set.}
    \label{tab:calibratingod}
    \begin{tabular}{|c|c||c|c|c||c|c|} \hline
    \multirow{2}{*}{Detector}&Calibration&\multicolumn{3}{|c|}{top-100 survival}&\multicolumn{2}{|c|}{thresholding} \\ \cline{3-7}
     &Method&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{laECE}$&$\mathrm{LRP}$&$\mathrm{laECE}$\\ \hline 
    \multirow{4}{*}{F R-CNN}& \xmark&$\mathbf{27.0}$&$\mathbf{77.9}$&$17.3$&$\mathbf{74.7}$&$43.3$\\
    &LR&$\mathbf{27.0}$&$\mathbf{77.9}$&$5.5$&$\mathbf{74.7}$&$17.7$\\
    &HB&$25.5$&$78.1$&$3.8$&$\mathbf{74.7}$&$18.6$\\
    &IR&$26.5$&$78.2$&$\mathbf{3.6}$&$\mathbf{74.7}$&$\mathbf{16.9}$\\
 \hline
     \multirow{4}{*}{RS R-CNN}& \xmark&$\mathbf{28.6}$&$\mathbf{76.8}$&$45.6$&$\mathbf{73.6}$&$32.0$\\
    &LR&$\mathbf{28.6}$&$\mathbf{76.8}$&$5.9$&$\mathbf{73.6}$&$17.4$\\
    &HB&$21.6$&$78.6$&$1.6$&$\mathbf{73.6}$&$19.6$\\
    &IR&$27.9$&$77.1$&$\mathbf{1.5}$&$\mathbf{73.6}$&$\mathbf{17.2}$\\
 \hline 
     \multirow{4}{*}{ATSS}& \xmark&$\mathbf{28.8}$&$\mathbf{76.7}$&$8.5$&$\mathbf{74.0}$&$\mathbf{15.7}$\\
    &LR&$\mathbf{28.8}$&$\mathbf{76.7}$&$3.6$&$\mathbf{74.0}$&$16.8$\\
    &HB&$23.8$&$77.9$&$1.7$&$74.1$&$18.7$\\
    &IR&$28.2$&$77.0$&$\mathbf{1.6}$&$\mathbf{74.0}$&$16.7$\\
 \hline 
     \multirow{4}{*}{D-DETR}& \xmark&$\mathbf{30.5}$&$\mathbf{75.5}$&$9.9$&$\mathbf{71.9}$&$15.9$\\
    &LR&$\mathbf{30.5}$&$\mathbf{75.5}$&$3.8$&$\mathbf{71.9}$&$\mathbf{15.7}$\\
    &HB&$23.7$&$77.2$&$1.5$&$\mathbf{71.9}$&$17.7$\\
    &IR&$29.8$&$75.8$&$\mathbf{1.4}$&$\mathbf{71.9}$&$15.9$\\
 \hline 
    \end{tabular}
\end{table}
}
\blockcomment{
\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.3em}
    \small
    \caption{Calibrating object detectors. \xmark: No calibration, HB: Histogram binning, IR: Isotonic Regresssion, LR: Linear Regression}
    \label{tab:calibratingod}
    \begin{tabular}{|c|c||c|c|c|c|c|c||c|c|c|c|} \hline
    \multirow{3}{*}{Detector}&\multirow{3}{*}{Calibration}&\multicolumn{6}{|c|}{top-100 survival}&\multicolumn{4}{|c|}{thresholding} \\ \cline{3-12}
    & &\multicolumn{3}{|c|}{COCO minival}&\multicolumn{3}{|c|}{Gen-OD  test}&\multicolumn{2}{|c|}{COCO val}&\multicolumn{2}{|c|}{Gen-OD test}\\ \cline{3-12}
     & &$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{laECE} $&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{laECE}$&$\mathrm{LRP}$&$\mathrm{laECE}$&$\mathrm{LRP}$&$\mathrm{laECE}$\\ \hline 
    \multirow{4}{*}{F R-CNN}& \xmark&$39.9$&$67.9$&$26.1$&$\mathbf{27.0}$&$\mathbf{77.9}$&$17.3$&$\mathbf{61.1}$&$26.1$&$\mathbf{74.7}$&$43.3$\\
    &LR&$39.9$&$67.5$&$4.3$&$\mathbf{27.0}$&$\mathbf{77.9}$&$5.5$&$\mathbf{61.1}$&$7.5$&$\mathbf{74.7}$&$17.7$\\
    &HB&$39.4$&$67.4$&$\mathbf{0.0}$&$25.5$&$78.1$&$3.8$&$\mathbf{61.1}$&$0.6$&$\mathbf{74.7}$&$18.6$\\
    &IR&$\mathbf{40.6}$&$\mathbf{67.1}$&$\mathbf{0.0}$&$26.5$&$78.2$&$\mathbf{3.6}$&$\mathbf{61.1}$&$\mathbf{0.0}$&$\mathbf{74.7}$&$\mathbf{16.9}$\\
 \hline
     \multirow{4}{*}{RS R-CNN}& \xmark&$42.0$&$66.0$&$41.9$&$\mathbf{28.6}$&$\mathbf{76.8}$&$45.6$&$\mathbf{59.6}$&$16.7$&$\mathbf{73.6}$&$32.0$\\
    &LR&$42.0$&$66.0$&$4.4$&$\mathbf{28.6}$&$\mathbf{76.8}$&$5.9$&$\mathbf{59.6}$&$7.3$&$\mathbf{73.6}$&$17.4$\\
    &HB&$35.6$&$67.9$&$\mathbf{0.0}$&$21.6$&$78.6$&$1.6$&$\mathbf{59.6}$&$0.3$&$\mathbf{73.6}$&$19.6$\\
    &IR&$\mathbf{42.7}$&$\mathbf{65.5}$&$\mathbf{0.0}$&$27.9$&$77.1$&$\mathbf{1.5}$&$\mathbf{59.6}$&$\mathbf{0.0}$&$\mathbf{73.6}$&$\mathbf{17.2}$\\
 \hline 
     \multirow{4}{*}{ATSS}& \xmark&$42.8$&$65.7$&$7.7$&$\mathbf{28.8}$&$\mathbf{76.7}$&$8.5$&$\mathbf{60.2}$&$18.3$&$\mathbf{74.0}$&$\mathbf{15.7}$\\
    &LR&$42.8$&$65.7$&$2.5$&$\mathbf{28.8}$&$\mathbf{76.7}$&$3.6$&$\mathbf{60.2}$&$7.7$&$\mathbf{74.0}$&$16.8$\\
    &HB&$38.4$&$67.1$&$\mathbf{0.0}$&$23.8$&$77.9$&$1.7$&$\mathbf{60.2}$&$0.5$&$74.1$&$18.7$\\
    &IR&$\mathbf{43.6}$&$\mathbf{65.2}$&$\mathbf{0.0}$&$28.2$&$77.0$&$\mathbf{1.6}$&$\mathbf{60.2}$&$\mathbf{0.0}$&$\mathbf{74.0}$&$16.7$\\
 \hline 
     \multirow{4}{*}{D-DETR}& \xmark&$44.3$&$64.2$&$7.8$&$\mathbf{30.5}$&$\mathbf{75.5}$&$9.9$&$\mathbf{57.2}$&$11.2$&$\mathbf{71.9}$&$15.9$\\
    &LR&$44.3$&$64.2$&$2.5$&$\mathbf{30.5}$&$\mathbf{75.5}$&$3.8$&$\mathbf{57.2}$&$7.2$&$\mathbf{71.9}$&$\mathbf{15.7}$\\
    &HB&$38.0$&$66.4$&$\mathbf{0.0}$&$23.7$&$77.2$&$1.5$&$\mathbf{57.2}$&$0.6$&$\mathbf{71.9}$&$17.7$\\
    &IR&$\mathbf{45.1}$&$\mathbf{63.7}$&$\mathbf{0.0}$&$29.8$&$75.8$&$\mathbf{1.4}$&$\mathbf{57.2}$&$\mathbf{0.0}$&$\mathbf{71.9}$&$15.9$\\
 \hline 
    %\hline
    %\multirow{2}{*}{NLL R-CNN}& &$40.1$&&$7.72$&$26.9$&&$8.86$\\
    %&HB&$40.1$&&&$26.8$&&\\ \hline
    %\multirow{2}{*}{ES R-CNN}& &$40.6$&&$7.89$&$27.2$&&$9.91$\\
    %&HB&$40.3$& & &$27.2$&& \\ \hline
    \end{tabular}
\end{table*}
}
%

\blockcomment{
    \textbf{The effect of covariate shift.}  Table \ref{tab:corr_calibration}
    \begin{table}
        \centering
        \small
        \setlength{\tabcolsep}{0.03em}
        \caption{Effect of corruptions on calibration.}
        \label{tab:corr_calibration}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|} \hline
             \multirow{2}{*}{Detector}&\multicolumn{4}{|c|}{COCO \textit{minival}}&\multicolumn{4}{|c|}{Gen-OD  \textit{test}}\\ \cline{2-9}
             &Clean&Sev. 1&Sev. 3&Sev. 5&Clean&Sev. 1&Sev. 3&Sev. 5 \\ \hline
        F R-CNN&$15.11$&$13.67$&$11.88$&$10.87$&$17.25$&$15.93$&$14.63$&$13.56$\\
        RS R-CNN&$41.90$&$42.00$&$41.83$&$41.01$&$45.59$&$45.34$&$44.83$&$43.54$\\
        ATSS&$7.69$&$7.30$&$6.86$&$6.37$&$8.52$&$8.34$&$8.07$&$7.40$\\
        D-DETR&$7.77$&$7.78$&$7.89$&$8.02$&$9.94$&$9.90$&$9.83$&$9.59$\\ \hline
        \end{tabular}
    \end{table}
}

%
% \paragraph{Discussions.}
%

%
% \textbf{Design Choices.} Using different number of bins. Different TP validation thresholds. See Supp.Mat
%

%
% \textbf{On false negatives.} One can assume that false negatives are detections with $\hat{p}_{i} = 0$ while computing the detection calibration error. Basides, in the extreme case, any possible bounding box without a detection can be considered as a detection with $\hat{p}_{i} = 0$. Since including such many detections may manipulate the expected calibration error by resulting in the first bin to dominate, we only use the detections obtained from the detector.
%
%
\blockcomment{
    \begin{figure*}[ht]
            \captionsetup[subfigure]{}
            \centering
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/faster_rcnn_r50_fpn_straug_3x_coco_severity_0_reliabilitydiagram.pdf}
            \caption{F R-CNN on COCO \textit{minival}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/rs_faster_rcnn_r50_fpn_straug_3x_coco_severity_0_reliabilitydiagram.pdf}
            \caption{RS R-CNN on COCO \textit{minival}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/atss_r50_fpn_straug_3x_coco_severity_0_reliabilitydiagram.pdf}
            \caption{ATSS on COCO \textit{minival}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/deformable_detr_r50_16x2_50e_coco_severity_0_reliabilitydiagram.pdf}
            \caption{D-DETR on COCO \textit{minival}}
            \end{subfigure}
    
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_reliabilitydiagram.pdf}
            \caption{F R-CNN on Gen-OD  \textit{test}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/rs_faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_reliabilitydiagram.pdf}
            \caption{RS R-CNN on Gen-OD  \textit{test}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/atss_r50_fpn_straug_3x_robustodgenod_severity_0_reliabilitydiagram.pdf}
            \caption{ATSS on Gen-OD  \textit{test}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/deformable_detr_r50_16x2_50e_robustodgenod_severity_0_reliabilitydiagram.pdf}
            \caption{D-DETR on Gen-OD  \textit{test}}
            \end{subfigure}
    
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_reliabilitydiagram.pdf}
            \caption{F R-CNN on Gen-OD  \textit{test}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/rs_faster_rcnn_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_reliabilitydiagram.pdf}
            \caption{RS R-CNN on Gen-OD  \textit{test}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/atss_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_reliabilitydiagram.pdf}
            \caption{ATSS on Gen-OD  \textit{test}}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms/deformable_detr_r50_16x2_50e_robustodgenod_severity_0_isotonic_regression_reliabilitydiagram.pdf}
            \caption{D-DETR on Gen-OD  \textit{test}}
            \end{subfigure}
            \caption{\textbf{(a)} 
            \textbf{(b)} }
            \label{fig:reliabilityhist}
    \end{figure*}
}
%
\blockcomment{
    \begin{figure*}[ht]
            \captionsetup[subfigure]{}
            \centering
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_coco_severity_0_identity_ap_style_reliabilitydiagram.pdf}
            \caption{uncalibrated \& top-100}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_coco_severity_0_isotonic_regression_ap_style_reliabilitydiagram.pdf}
            \caption{calibrated \& top-100}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_coco_severity_0_identity_thresholding_reliabilitydiagram.pdf}
            \caption{uncalibrated \& thresholded}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_coco_severity_0_isotonic_regression_thresholding_reliabilitydiagram.pdf}
            \caption{calibrated \& thresholded}
            \end{subfigure}
    
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_identity_ap_style_reliabilitydiagram.pdf}
            \caption{uncalibrated \& top-100}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_ap_style_reliabilitydiagram.pdf}
            \caption{calibrated \& top-100}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_identity_thresholding_reliabilitydiagram.pdf}
            \caption{uncalibrated \& thresholded}
            \end{subfigure}
            \begin{subfigure}[b]{0.24\textwidth}
            \includegraphics[width=\textwidth]{Images/histograms_2/atss_r50_fpn_straug_3x_robustodgenod_severity_0_isotonic_regression_thresholding_reliabilitydiagram.pdf}
            \caption{calibrated \& thresholded}
            \end{subfigure}
            \caption{ATSS. Upper row: val set, lower row: test set }
            \label{fig:atssreliabilityhist}
    \end{figure*}
}
%
\blockcomment{
\begin{table}
    \centering
    \setlength{\tabcolsep}{0.15em}
    \small
    \caption{Calibrating object detectors. \xmark: No calibration, HB: Histogram binning, IR: Isotonic Regresssion, LR: Linear Regression}
    \label{tab:calibrate_based_on_topk}
    \begin{tabular}{|c|c||c|c|c|c|c|c|} \hline
    \multirow{2}{*}{Detector}&\multirow{2}{*}{Method}&\multicolumn{3}{|c|}{COCO minival}&\multicolumn{3}{|c|}{Gen-OD  test}\\ \cline{3-8}
     & &$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{laECE} $&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{laECE}$\\ \hline 
    \multirow{4}{*}{F R-CNN}& \xmark&$39.9$&$67.9$&$26.08$&$\mathbf{27.0}$&$\mathbf{77.9}$&$17.25$\\
    &LR&$39.9$&$67.5$&$4.28$&$\mathbf{27.0}$&$\mathbf{77.9}$&$5.53$\\
    &HB&$39.4$&$67.4$&$\mathbf{0.00}$&$25.5$&$78.1$&$3.83$\\
    &IR&$\mathbf{40.6}$&$\mathbf{67.1}$&$\mathbf{0.00}$&$26.5$&$78.2$&$\mathbf{3.63}$\\
    \hline
    \multirow{4}{*}{RS R-CNN}& \xmark&$42.0$&$66.0$&$41.90$&$\mathbf{28.6}$&$\mathbf{76.8}$&$45.59$\\
    &LR&$42.0$&$66.0$&$4.43$&$\mathbf{28.6}$&$\mathbf{76.8}$&$5.92$\\
    &HB&$35.6$&$67.9$&$\mathbf{0.00}$&$21.6$&$78.6$&$1.58$\\
    &IR&$\mathbf{42.7}$&$\mathbf{65.5}$&$\mathbf{0.00}$&$27.9$&$77.1$&$\mathbf{1.51}$\\ 
 \hline
    \multirow{4}{*}{ATSS}&\xmark&$42.8$&$65.7$&$7.69$&$\mathbf{28.8}$&$\mathbf{76.7}$&$8.52$\\
    &LR&$42.8$&$65.7$&$2.53$&$\mathbf{28.8}$&$\mathbf{76.7}$&$3.56$\\
    &HB&$38.4$&$67.1$&$\mathbf{0.00}$&$23.8$&$77.9$&$1.65$ \\
    &IR&$\mathbf{43.6}$&$\mathbf{65.2}$&$\mathbf{0.00}$&$28.2$&$77.0$&$\mathbf{1.58}$ \\
\hline
    \multirow{4}{*}{D-DETR}&\xmark&$44.3$&$64.2$&$7.77$&$\mathbf{30.5}$&$\mathbf{75.5}$&$9.94$\\
    &LR&$44.3$&$64.2$&$2.45$&$\mathbf{30.5}$&$\mathbf{75.5}$&$3.75$\\
    &HB&$38.0$&$66.4$&$\mathbf{0.00}$&$23.7$&$77.2$&$1.51$\\ 
    &IR&$\mathbf{45.1}$&$\mathbf{63.7}$&$\mathbf{0.00}$&$29.8$&$75.8$&$\mathbf{1.39}$\\ 
 \hline 
    \end{tabular}
\end{table}
%
\begin{table*}
    \centering
    \setlength{\tabcolsep}{0.15em}
    \small
    \caption{Calibrating object detectors. \xmark: No calibration, HB: Histogram binning, IR: Isotonic Regresssion, LR: Linear Regression}
    \label{tab:calibrate_based_lrp_opt}
    \begin{tabular}{|c|c||c|c|c|c|c|c|c|c|c|c|} \hline
    \multirow{2}{*}{Detector}&\multirow{2}{*}{Method}&\multicolumn{5}{|c|}{COCO minival}&\multicolumn{5}{|c|}{Gen-OD  test}\\ \cline{3-12}
     & &$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{LRP_{0.1}}$&$\mathrm{laECE}$&$\mathrm{mMCE}$&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{LRP_{0.1}}$&$\mathrm{laECE}$&$\mathrm{mMCE}$\\ \hline 
    \multirow{4}{*}{F R-CNN}& \xmark&$34.6$&$67.9$&$61.1$&$26.1$&$52.5$&$23.6$&$78.1$&$74.7$&$43.3$&$57.8$\\
    &LR&$34.6$&$67.9$&$61.1$&$7.5$&$32.9$&$23.6$&$78.1$&$74.7$&$17.7$&$33.8$\\
    &HB&$35.6$&$67.4$&$61.1$&$0.6$&$4.7$&$22.4$&$78.5$&$74.7$&$18.6$&$39.8$\\
    &IR&$35.1$&$67.6$&$61.1$&$0.0$&$0.0$&$23.2$&$78.4$&$74.7$&$16.9$&$49.6$\\
 \hline 
     \multirow{4}{*}{ATSS}& \xmark&$36.7$&$66.2$&$60.2$&$18.3$&$37.0$&$24.8$&$77.0$&$74.0$&$15.7$&$32.8$\\
    &LR&$36.7$&$66.2$&$60.2$&$7.7$&$25.8$&$24.8$&$77.0$&$74.0$&$16.8$&$34.3$\\
    &HB&$37.7$&$65.6$&$60.2$&$0.5$&$4.4$&$23.6$&$77.2$&$74.1$&$18.7$&$38.5$\\
    &IR&$37.3$&$65.8$&$60.2$&$0.0$&$0.0$&$24.5$&$77.1$&$74.0$&$16.7$&$54.9$\\
 \hline 
     \multirow{4}{*}{RS R-CNN}& \xmark&$36.3$&$66.4$&$59.6$&$16.7$&$38.5$&$24.8$&$77.0$&$73.6$&$32.0$&$50.2$\\
    &LR&$36.3$&$66.4$&$59.6$&$7.3$&$26.6$&$24.8$&$77.0$&$73.6$&$17.4$&$34.9$\\
    &HB&$37.2$&$65.9$&$59.6$&$0.3$&$2.9$&$23.7$&$77.3$&$73.6$&$19.6$&$40.1$\\
    &IR&$36.8$&$66.1$&$59.6$&$0.0$&$0.0$&$24.4$&$77.2$&$73.6$&$17.2$&$52.9$\\
 \hline 
     \multirow{4}{*}{D-DETR}& \xmark&$38.2$&$64.5$&$57.2$&$11.2$&$28.6$&$26.3$&$75.6$&$71.9$&$15.9$&$28.4$\\
    &LR&$38.2$&$64.5$&$64.5$&$7.2$&$27.6$&$26.3$&$75.6$&$71.9$&$15.7$&$31.5$\\
    &HB&$39.3$&$63.9$&$57.2$&$0.6$&$4.7$&$25.1$&$75.9$&$71.9$&$17.7$&$37.0$\\
    &IR&$38.8$&$64.2$&$57.2$&$0.0$&$0.0$&$25.9$&$75.9$&$71.9$&$15.9$&$53.2$\\
 \hline 
    %\hline
    %\multirow{2}{*}{NLL R-CNN}& &$40.1$&&$7.72$&$26.9$&&$8.86$\\
    %&HB&$40.1$&&&$26.8$&&\\ \hline
    %\multirow{2}{*}{ES R-CNN}& &$40.6$&&$7.89$&$27.2$&&$9.91$\\
    %&HB&$40.3$& & &$27.2$&& \\ \hline
    \end{tabular}
\end{table*}
%
Accordingly, the performance measure, which is to be compared against the joint confidence score $\hat{p}_i$, needs to capture the performance in terms of both classification (e.g. accuracy for classification in Eq. \eqref{eq:classifiercalibration}) and localisation (e.g. mean squared error for regression in Eq. \eqref{eq:regressioncalibration}). 
%
To be aligned with the practical usage, we use the final predictions by matching them following the performance measures (Section \ref{subsec:objectdetectors}).
%
Note that, this is different from, e.g., Kuppers et al. \cite{mvcalibrationod} matching all overlapping detections with the objects while focusing only on the localisation aspect of the calibration. 

\textbf{Definition.} After matching the detections with the objects (Section \ref{sec:relatedwork}), calibration error for class $c_i$ can be evaluated by:
%
\begin{align}\label{eq:calibration}
    \mathbb{E}[ \lvert \hat{p}_{i} - \zeta(\mathcal{D}, \mathcal{G}) \rvert ],
\end{align}
%
where $\mathcal{D}$ and $\mathcal{G}$ is the detection and ground truth sets for class $c_i$, and $\zeta(\cdot,\cdot)$ is a higher-better scoring function jointly evaluating classification and localisation performances, which is similar to $\hat{p}_{i}$. 
%
In particular, we define $\zeta(\cdot,\cdot)$ as the product of precision ($\mathbb{P}(c_i = \hat{c}_i | \hat{p}_{i})$) and the expected normalized localisation quality of true positives ($\mathbb{E}(\mathrm{lq(i)} | \hat{p}_{i}))$) \KO{Discussion point. 
%
Should we include false negatives in $\zeta(\cdot,\cdot)$?} yielding,
%
\begin{align}\label{eq:calibration_od}
    \mathbb{E}[ \lvert \hat{p}_{i} - \mathbb{P}(c_i = \hat{c}_i | \hat{p}_{i}) \mathbb{E}(\mathrm{lq(i)} | \hat{p}_{i})) \rvert ].
\end{align}
%
We normalize the localisation qualities between $[0,1]$ to align their range with that of $\hat{p}_{i}$ and use the product of the classification and localisation performance to be aligned with how $\hat{p}_{i}$ should be obtained: Assuming the independence of classification and localisation predictions following existing detectors; $\hat{p}_{i}=\hat{p}_{i}^{cls} \times \hat{p}_{i}^{loc}$ such that $\hat{p}_{i}^{cls}$ and $\hat{p}_{i}^{loc}$ are the confidence scores for classification and localisation. 
%
The localisation confidence score can be seen as a decreasing function of the variance of the predictive distribution ($f_{\hat{B}_i}(b)$) to match the actual localisation quality of the bounding box, which is, in fact, directly predicted by several SOTA methods \cite{IoUNet,paa} for increasing the accuracy, but not the calibration. 
%
As a result, Eq. \ref{eq:calibration_od} suggests that \textit{for a calibrated detector, the detection confidence score should be equal to the product of precision and localisation quality.}
%
%employ the square root of the individual performance indicators to for two reasons: First, it prevents the scores to have a bias towards low values and second with certain assumptions we can show that if classification and localisation tasks are perfectly calibrated, then Eq. \ref{eq:calibration_od} will yield $0$ (see calibration errors of individual tasks for more discussion). Overall, Eq. \eqref{eq:calibration_od} can be interpreted as \textit{the confidence of the predictions should match the geometric mean of precision and localisation quality}. Supp.Mat presents the relation of $\zeta(\cdot, \cdot)$ with precision and LRP Error (Section \ref{sec:relatedwork}). Finally, to obtain the calibration error in the detector-level, we average over the class-wise calibration errors by ignoring a class if it does not have any prediction. 
%
Calibration of a model is defined as the alignment of the performance of the model and its confidence \cite{calibration,FocalLoss_Calibration}, i.e., formally,
%
\begin{align}
  \label{eq:calibration}
  \int_{\hat{p}} \lvert  \mathrm{performance}(\hat{y}, y) - \hat{p}  \rvert d \hat{p},
\end{align}
%
such that $\mathrm{performance}(\hat{y}, y)$ measures the model performance given predictions $\hat{y}$ and ground truths $y$, and $\hat{p}$ is the predicted confidence scores. 
%
Accordingly, the underlying $\mathrm{performance}(\cdot, \cdot)$ should be a high-better measure and consistently account for all aspects of the model performance, which involves \textit{both} classification and localisation performances for object detection and has not been properly investigated from this perspective. 
%
Accordingly, our main idea for calibration of object detectors is inspired by the observation that \textit{the more confident the visual detector is, the better classification and localisation performance one should expect} (Fig. x). 
%
Note that in such a setting, the detection confidence score is expected to account for both classification and localisation, which also aligns with the recent studies \cite{IoUNet,FCOS,ATSS,GFL,GFLv2,varifocalnet,aLRPLoss,RSLoss} to unify classification and localisation scores to improve the accuracy of the model.
%
For simplicity, we assume that there is a single ID class, and then, as commonly employed by the performance measures of object detection \cite{PASCAL,PanopticSegmentation,COCO,LRPPAMI} we average over the class-wise calibration errors to obtain the calibration error of the detector. 
%
\subsection{Calibration Criteria and Errors for Individual Tasks}
This section derives classification and localisation calibration errors:
%
\textbf{Classification calibration criterion and error.} The precision of a detector should match the confidence of the object detector, i.e.,
%
\begin{align}\label{eq:precision}
    \mathrm{pr}(\hat{\mathbb{D}}, m(\hat{\mathbb{D}})) = \frac{\mathrm{TP}(m(\hat{\mathbb{D}}))}{D}=\hat{p},
\end{align}
%
where the number of true positive can be estimated using the assignments over all detections as $\mathrm{TP}(m(\hat{\mathbb{D}})) = \sum_{i=1}^D [m(\hat{d}_i) \neq \O]$ with $[\cdot]$ being the indicator function. 
%
Then, similar to Fabian et al. \cite{CalibrationOD}, by replacing $\mathrm{performance}(\hat{y}, y)$ in Eq. \eqref{eq:calibration} by $\mathrm{pr}(\hat{\mathbb{D}}, m(\hat{\mathbb{D}}))$, approximating the integral by discretizing the probability space into $B$ equally spaced bins and partitioning $\hat{\mathbb{D}}$ into those bins, i.e., $\hat{\mathbb{D}}=\bigcup_{i=1}^B \hat{\mathbb{D}}_i$, one can obtain classification and localisation calibration performances of the visual detector respectively. 
%
Specifically; expected object detection calibration error for classification is defined as,
%
\begin{align}
  \label{eq:clscalibration}
   \mathrm{ECE}_{OD}^{cls} = \sum_{i=1}^B \frac{|\hat{\mathbb{D}}_i|}{|\hat{\mathbb{D}}|} \lvert \mathrm{pr}(\hat{\mathbb{D}}_i, m(\hat{\mathbb{D}}_i)) - \hat{p}(\hat{\mathbb{D}}_i)  \rvert,
\end{align}
%
where $\hat{p}(\hat{\mathbb{D}}_i) = \frac{1}{|\hat{\mathbb{D}}_i|} \sum_{\{\hat{b}_i, \hat{p}_i\} \in \hat{\mathbb{D}}_i} \hat{p}_i $
%
\textbf{localisation calibration criterion and error.} Normalized average IoUs of true positives, denoted by $\Bar{\mathrm{IoU}}(\hat{\mathbb{D}}, m(\hat{\mathbb{D}}))$ and defined as,
%
\begin{align}\label{eq:avgIoU}
    \frac{1}{\mathrm{TP}(m(\hat{\mathbb{D}}))} \sum_{i=1}^{|\hat{\mathbb{D}}|} [m(\hat{d}_i)) \neq \O] \frac{\mathrm{IoU}(\hat{b}_i, m(\hat{d}_i)) -\tau}{1-\tau},
\end{align}
%
should match the confidence of the object detector confidence, $\Bar{\mathrm{IoU}}(\hat{\mathbb{D}}, m(\hat{\mathbb{D}})) = \hat{p}$. 
%
We employ the normalize the IoU values considering that the range of the scores is $[0,1]$ but that of IoUs is $[\tau,1]$. 
%
Then, similar to classification, we define expected object detection calibration for localisation as,
\begin{align}
  \label{eq:loccalibration}
  \mathrm{ECE}_{OD}^{loc} = \sum_b \frac{\mathrm{TP}(m(\hat{\mathbb{D}}_i))}{\mathrm{TP}(m(\hat{\mathbb{D}}))} \lvert \Bar{\mathrm{IoU}}(\hat{\mathbb{D}}_i, m(\hat{\mathbb{D}}_i)) - \hat{p}(\hat{\mathbb{D}}_i)  \rvert.
\end{align}
%
\subsection{Object Detection Calibration Criterion and Error [OPTION 1: RELAXING THE TIGHT CONSTRAINTS OF COMPONENTS BUT PRESERVING THE AVERAGE]}
%
Next, we develop a performance measure given precision (Eq. \ref{eq:precision}) and normalized average IoUs (Eq. \ref{eq:avgIoU}) in order to measure the calibration performance of an object detector. 
%
While these two quantities can be combined by different functions as long as the employed function (i) is an increasing function of these two and (ii) yields a value between these two, we employ their geometric mean owing to the resulting intuitive formulation and relation with existing performance measures,
%
\begin{align}
  \label{eq:calibrationOD}
   & \sqrt{\mathrm{pr}(\hat{\mathbb{D}}, m(\hat{\mathbb{D}})) \times \Bar{\mathrm{IoU}}(\hat{\mathbb{D}}, m(\hat{\mathbb{D}}))}, \\
   \label{eq:odcalibrationcriterion}
  = & \sqrt{\underbrace{\frac{1}{|\hat{\mathbb{D}}|} \sum_{i=1}^{|\hat{\mathbb{D}}|} [m(\hat{d}_i)) \neq \O] \frac{\mathrm{IoU}(\hat{b}_i, m(\hat{d}_i)) -\tau}{1-\tau}}_{\mathrm{pr}_{IoU}(\hat{\mathbb{D}}_i, m(\hat{\mathbb{D}})_i)}}.
\end{align}
%
Note that the expression inside the square-root operation corresponds to summing over the normalized IoUs of true positives and normalizing it by the number of all detections, which is very similar to precision, which, in fact, adds $1$ (instead of the normalized IoU of the true positive) to the nominator. 
%
Therefore, we define that expression as \textit{IoU-weighted precision}, $\mathrm{pr}_{IoU}(\hat{\mathbb{D}}, m(\hat{\mathbb{D}}))$ (see also Supp.Mat. for the relation of IoU-weighted precision with LRP Error). 
%
Expecting that Eq. \eqref{eq:odcalibrationcriterion} to match $\hat{p}_i$, we define expected object detection calibration error as follows:
%
\begin{align}
  \label{eq:odcalibration}
   \mathrm{ECE}_{OD} = \sum_{i=1}^B \frac{|\hat{\mathbb{D}}_i|}{|\hat{\mathbb{D}}|} \lvert \sqrt{\mathrm{pr}_{IoU}(\hat{\mathbb{D}}_i, m(\hat{\mathbb{D}}_i))} - \hat{p}(\hat{\mathbb{D}}_i)  \rvert.
\end{align}
%
Note that, our proposed calibration errors (i) evaluate classification, localisation and object detection calibration performances, (ii) facilitate leveraging existing analysis tools developed for classification, e.g. reliability diagrams \cite{calibration}.
%

%
\textbf{Advantages of Option 1 :}
\begin{itemize}
    \item $\mathrm{ECE}_{OD}$ only expects the geometric average of classification and localisation performances to be calibrated. Hence, in practice, it does not enforce both of the strict calibration criteria (i.e., both for classification and localisation) at once.
    \item $\mathrm{ECE}_{OD}$ is still a calibration measure (following Eq. \ref{eq:calibration}). That's why, associated calibration tools such as the reliability diagrams can be used.
\end{itemize}
%
\textbf{Disadvantages of Option 1 :}
\begin{itemize}
    \item $\mathrm{ECE}_{OD}$ is not necessarily between $\mathrm{ECE}_{OD}^{loc}$ and $\mathrm{ECE}_{OD}^{cls}$.
\end{itemize}
%
\subsection{Object Detection Calibration Criterion and Error [OPTION 1: KEEPING THE TIGHT CONSTRAINTS]}
%
\begin{align}
  \label{eq:odcalibration2}
   \mathrm{ECE}_{OD} = \frac{2 \times \mathrm{ECE}_{OD}^{loc} \times \mathrm{ECE}_{OD}^{cls}}{\mathrm{ECE}_{OD}^{loc} + \mathrm{ECE}_{OD}^{cls}} 
\end{align}
%
Note that, our proposed calibration errors (i) evaluate classification, localisation and object detection calibration performances, (ii) facilitate leveraging existing analysis tools developed for classification, e.g. reliability diagrams \cite{calibration}.
%
\blockcomment{
    \textbf{Classification Calibration Error.} Following our discussion for the joint distribution, one can similarly define the calibration errors for marginal distributions $f_{C_i}(c)$ and $f_{B_i}(b)$. 
    %
    Accordingly, the classification calibration error is,
    %
    \begin{align}\label{eq:odclscalibration}
        \mathbb{E}[ \lvert \hat{p}_{i}^{cls} - \mathbb{P}(C_i = \hat{c}_i | \hat{p}_{i}^{cls}) \rvert ],
    \end{align}
    %
    \textbf{localisation Calibration Error.} The localisation calibration error is defined as,
    %
    \begin{align}
    \label{eq:odloccalibration}
        \mathbb{E}[ \lvert \hat{p}_{i}^{loc} - \mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i}^{loc})| \hat{p}_{i}^{loc}) \rvert ].
    \end{align}
    %
    Note that, if spearman correlation between $\hat{p}_{i}^{cls}$s and $\hat{p}_{i}^{reg}$s is $1$; Eq. \eqref{eq:calibrationindependence} is minimized when both classification and localisation tasks are perfectly calibrated (see Supp.Mat. for the proof). 
}
%
% \subsection{Practical Usage}
%
%
\textbf{Advantages of Option 2 :}
\begin{itemize}
    \item Harmonic mean (or any mean) enforces $\mathrm{ECE}_{OD}$ to be between $\mathrm{ECE}_{OD}^{loc}$ and $\mathrm{ECE}_{OD}^{cls}$.
\end{itemize}
%

%
\textbf{Disadvantages of Option 2 :}
\begin{itemize}
        \item $\mathrm{ECE}_{OD}$ is not a calibration measure defined by Eq. \ref{eq:calibration}.
        \item Enforcing Eq. \ref{eq:precision} and Eq. \ref{eq:avgIoU} based on $\hat{p}$ may be too strict. 
\end{itemize}
%
\subsection{Are Common Object Detectors Calibrated?}
%
\begin{table}
    \centering
    \small
    \caption{Calibration performance of different object detectors.}
    \label{tab:calibration}
    \begin{tabular}{|c||c|c|c|} \hline
    Detector&$\mathrm{ECE}_{OD}$&$\mathrm{ECE}_{OD}^{cls}$&$\mathrm{ECE}_{OD}^{loc}$\\ \hline
    Faster R-CNN \cite{FasterRCNN}& & &\\
    RS-R-CNN \cite{RSLoss}& & &   \\
    ATSS \cite{ATSS}& & &   \\
    D-DETR \cite{DDETR}& & & \\ \hline
    \end{tabular}
\end{table}

\textbf{Does using an explicit $\hat{p}_{i}^{loc}$ improve calibration?} Table \ref{tab:p_loceffect} -10 and 30 for both
%
\begin{table}
    \centering
    \setlength{\tabcolsep}{0.2em}
    \small
    \caption{Combining localisation and Classification Uncertainty}
    \label{tab:p_loceffect}
    \begin{tabular}{|c|c||c|c|c|c|} \hline 
     \multirow{2}{*}{Detector}&\multirow{2}{*}{$\hat{p}_{i}$}&\multicolumn{2}{|c|}{COCO minival}&\multicolumn{2}{|c|}{RobustOD test}\\ \cline{3-6}
     &&$\mathrm{LRP}$&$\mathrm{laECE}$&$\mathrm{LRP}$&$\mathrm{laECE}$\\ \hline 
    %\multirow{4}{*}{ATSS}&\multirow{2}{*}{$\hat{p}_{i}^{cls}$}&&$60.6$&$12.5$&$73.6$&$16.0$\\
    %& &\cmark&$60.6$&$0.0$&$73.7$&$16.4$\\ \cline{2-7}
    %&\multirow{2}{*}{$\hat{p}_{i}^{cls} \times \hat{p}_{i}^{loc}$}&&$60.2$&$18.3$&$74.0$&$15.7$\\
    %& &\cmark&$60.2$&$0.0$&$74.0$&$16.7$\\ \hline \hline
    \multirow{2}{*}{NLL R-CNN}&$\hat{p}_{i}^{cls}$&$61.5$&$26.3$&$74.9$&$42.6$\\
    %& &$61.5$&$0.0$&$74.9$&$16.2$\\ \cline{2-6}
    &$\hat{p}_{i}^{cls} \times \hat{p}_{i}^{loc}$&$61.5$&$13.9$&$74.6$&$20.4$\\ \hline
    \multirow{2}{*}{ES R-CNN}&$\hat{p}_{i}^{cls}$&$61.1$&$25.9$&$74.5$&$43.4$\\
    %& &$61.5$&$0.0$&$74.9$&$16.2$\\ \cline{2-6}
    &$\hat{p}_{i}^{cls} \times \hat{p}_{i}^{loc}$&$61.1$&$11.8$&$75.2$&$23.6$\\
    %& &$61.4$&$0.1$&$74.6$&$17.4$\\ 
    \hline 
    \end{tabular}
\end{table}
}

\blockcomment{
\subsection{Localisation-aware ECE [Version 2]} \label{subsec:mECE}
%
% Here we introduce a core contribution of this work, the Object Detector ECE, termed laECE, which measures the calibration error for object detectors. 
%
Here we derive Localisation-aware ECE in which $\hat{p}_i$, the detection confidence score, accounts for both classification and localisation performance.
%
Before proceeding with our derivation, we note that obtaining $\hat{p}_i$ is still an open problem in object detection.
%
Specifically, while earlier detectors \cite{SSD,FasterRCNN,FocalLoss,RFCN} generally use classification confidence as $\hat{p}_i$, the recent ones \cite{IoUNet,KLLoss,FCOS,GFL,varifocalnet,GFLv2,aLRPLoss,RSLoss,RankDetNet,paa} tend to combine localisation and classification confidences in $\hat{p}_i$, which is shown to be effective for improving the accuracy.
%
To do so, while such methods use different ways, one common example is to train an additional auxiliary head to regress the localisation quality (e.g., IoU) of the predictions \cite{IoUNet,paa,FCOS,ATSS,KLLoss,maskscoring,yolact-plus}, which can be interpreted as the localisation confidence.
%
Then during inference, the predicted classification confidence is combined with the localisation confidence, e.g., through multiplication, so that $\hat{p}_i$ to represent the joint confidence.
%
In our derivation, we adopt this recent perspective, as it aligns with the joint nature of the object detection.
%
%
%Assuming $\hat{p}_i$ is a sample from the probability distribution $\mathcal{P}$,  we define the calibration error of $f_J(X)$ as

%Formulating the calibration from this joint perspective is nontrivial mainly due to two challenges: (C1) The design of the calibration criterion needs attention since a single $\hat{p}_i$ should consistently account for both classification and localisation calibration; and (C2) existing measures of calibration for classification and regression has different interpretations of the confidence, say $p$, as illustrated on \cref{fig:iouprob_approx}: while a higher $p$ implies better performance for classification \cite{calibration,AdaptiveECE,verifiedunccalibration,rethinkcalibration,FocalLoss_Calibration,calibratepairwise}, the regression calibration use credible intervals \cite{regressionunc,distributioncalibrationregression}, which, instead of shrinking for a better performance, enlarge and get away from the mode of the predictive distribution as $p$ increases. 
%
%Conversely for object detection, following the definition of calibration, we argue that the joint performance considering classification and localisation should increase as $\hat{p}_i$ increases to provide more useful information to subsequent decision systems.
%
%We next derive the calibration criterion by addressing (C1) and our approach to address (C2) will be discussed shortly.
%

\textbf{Derivation.} We assume a hypothetical object detector, $f_J(X)$, to yield a full joint distribution for each prediction: $f_J(X) = \{p_{C_i, B_i}(c, b)\}^N$ where $p_{C_i, B_i}(c, b)$ is the joint distribution of the random variables $C_i \in \{1, ..., K\}$ and $B_i \in \mathbb{R}^{4}$. 
%
Given $p_{C_i, B_i}(c, b)$, the $i$th detection ($\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$) can be recovered as the modes of the marginal distributions $p_{C_i}(c)$ and $p_{B_i}(b)$, with $\hat{p}_i$ obtained as above.
%
% The mode of the marginal distributions, $p_{C_i}(c)$ and $p_{B_i}(b)$, correspond to $\hat{c}_i$ and $\hat{b}_i$; the detection confidence score $\hat{p}_i$ corresponds to the confidence of the $i$th detection, which is obtained in different ways in practice as aforementioned. 
%
%To represent classification and localisation consistently by $\hat{p}_i$ and address (C1), considering that since $\hat{p}_i$ represents the confidence, not the credible interval, we start with the equivalent criterion for localisation which is $(1-\hat{p}_i)$\% of the ground truths should \textit{not} be within the $\hat{p}_i$ credible interval (compare with calibrated regressor in \cref{fig:iouprob_approx}).
%
%Besides, the probability should match $\hat{p}_i$ not $(1-\hat{p}_i)$; hence we simply rewrite the expression as $\hat{p}_i$\% of the ground truths should not be within the $1-\hat{p}_i$ credible interval.
%hence a higher $\hat{p}_i$ will shrink the credible interval to enforce better localisation performance.
%
Consequently, assuming $\hat{p}_i$ is a realization of the random variable $P_i$, we expect $f_J(X)$ to combine the properties of calibrated classifier and regressor as illustrated in \cref{fig:calibration_def}, hence it is perfectly calibrated if
%
{\small
\begin{align}\label{eq:gen_calibration}
    \mathbb{P}(C_i = \hat{c}_i, b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_i) | P_{i} = \hat{p}_i) = \hat{p}_i, \forall \hat{p}_i \in [0, 1],
\end{align}
}
%
such that $b_{\psi(i)}$ is the ground truth box that $i$th prediction matches with and $\mathcal{F}_{B_i}(\hat{p}_{i})$ is the set of boxes within the $\hat{p}_{i}$ credible region centered at $\hat{b}_i$ in the distribution $p_{B_i}(b)$.
%
App. \ref{app:calibration} provides the formal definition of $\mathcal{F}_{B_i}(\hat{p}_{i})$.
%
Then, the calibration error of $f_J(X)$ based on Eq. \eqref{eq:gen_calibration} is
%
{\small
\begin{align}\label{eq:calibration}
    \mathbb{E}_{P_{i}}[ \lvert \hat{p}_{i} - \mathbb{P}(C_i = \hat{c}_i, b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i}) | P_{i}=\hat{p}_i)) \rvert ],
\end{align}
}
%
% such that $b_{\psi(i)}$ is the ground truth box that $i$th prediction matches and $\mathcal{F}_{B_i}(\hat{p}_{i})$ is the set of boxes within the $1-\hat{p}_{i}$ confidence interval from $\hat{b}_i$ considering $p_{B_i}(b)$\footnote{We use confidence intervals for localisation, which is in fact a regression task, following Kuleshov et al.\cite{regressionunc}. App. \ref{app:subsec_cal_relation} presents the details.}. 
%
where we assume independence between classification and localisation, yielding
%
{\small
\begin{align}\label{eq:calibrationindependence}
    \mathbb{E}_{P_i}[ \lvert \hat{p}_{i} - \mathbb{P}(C_i = \hat{c}_i | P_{i}=\hat{p}_i) \mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i})| \hat{p}_{i}) \rvert ].
\end{align}
}
%
%and $\hat{p}_{i}$ can be expressed as, 
%
%\begin{align}\label{eq:score}
%    \hat{p}_{i} = \hat{p}_{i}^{cls} \times \hat{p}_{i}^{loc},
%\end{align}
%
%where $\hat{p}_{i}^{cls}$ and $\hat{p}_{i}^{loc}$ are the confidence scores for classification and localisation respectively. 
%
Note that Eq. \eqref{eq:calibrationindependence} consists of two terms:
%
(i) $\mathbb{P}(C_i = \hat{c}_i | P_{i}=\hat{p}_i)$ is the ratio of the number of correctly-classified detections ($\mathrm{N_{TP}}$) and the total number of detections ($\mathrm{N_{TP}} + \mathrm{N_{FP}}$), which is the precision;
%
(ii) $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i})| P_{i}=\hat{p}_i)$ represents the probability that the ground truth $b_{\psi(i)}$ is within a $\hat{p}_{i}$ credible region of $\hat{b}_i$; thereby representing the localisation quality of the prediction, which we explore more next.
%

\textbf{Practical Usage.} $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i})| P_{i}=\hat{p}_i)$ cannot be evaluated on common object detectors, which are not probabilistic, since such detectors directly predict $\hat{b}_i$ and hence $p_{B_i}(b)$ is not available.
%
Hence, considering that $\hat{p}_i$ should reflect the joint quality of the prediction to enable the subsequent systems to decide properly, in practice a performance measure for localisation is a suitable proxy of $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i})| P_{i}=\hat{p}_i)$.
%
With such a proxy, a higher precision or the localisation quality of a prediction require a higher $\hat{p}_i$ to minimize the error in Eq. \eqref{eq:calibrationindependence}, which is intuitive.
%
%Furthermore, even if the detector is a probabilistic, it can be hard to compute due to requiring evaluating a multivariate distribution.
%
%As an example, while $p_{B_i}(b)$ is represented by multivariate Gaussian with full covariance matrix (\cref{sec:relatedwork}) in \cite{RegressionUncOD}, only the diagonal elements of the covariance matrix are used during evaluation\cite{probdet}.
%
%
%Therefore, we exploit IoU, the common localisation quality, as a proxy for $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i})| P_{i}=\hat{p}_i)$.
%
In particular, we use the average IoU of TPs, enabling us to estimate the calibration error of any object detector only by relying on the conventional representation of the detections, i.e., $\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$.
%
Besides, we (i) compute the average calibration error over classes following performance measures in object detection \cite{COCO,LVIS,Objects365,OpenImages, LRPPAMI} to prevent more frequent classes to dominate the calibration error; and (ii) discretize the confidence score space into $J$ equally-spaced bins similar to \cite{calibration,verifiedunccalibration} by splitting the detections into these bins for each class ($J^{c}=25$ for class $c$) since the underlying integration of $\mathbb{E}_{P_{i}}[\cdot]$ is intractable.
%
Consequently, the calibration error for a class $c$, denoted by $\mathrm{LaECE}^c$, is given as the weighted average of the differences of the confidence score from the product of precision ($\mathrm{precision}^{c}(j)$) and average IoU of TPs ($\bar{\mathrm{IoU}}^{c}(j)$)
%
{\small
\begin{align}
\label{eq:odcalibrationfinal1}
   \mathrm{LaECE}^c 
   & = \sum_{j=1}^{J^{c}} \frac{|\hat{\mathcal{D}}^{c}_j|}{|\hat{\mathcal{D}}^{c}|} \left\lvert \bar{p}^{c}_{j} - \mathrm{precision}^{c}(j) \times \bar{\mathrm{IoU}}^{c}(j)  \right\rvert,
\end{align}}
%
where $\hat{\mathcal{D}}^{c}$ denotes the set of all detections, $\hat{\mathcal{D}}_j^{c}	\subseteq \hat{\mathcal{D}}^{c}$ is the set of detections in bin $j$ and $\bar{p}_{j}^{c}$ is the mean detection scores in bin $j$ for class $c$. 
%
Then, $\mathrm{LaECE}$ of an object detector is the average over $\mathrm{LaECE}^c$ for $c \in \{1, ..., K\}$.
%
Thus, we have presented a tractable approach to compute the calibration error accounting for both classification \emph{and} localisation.

%
% While $\mathbb{P}(b_{\psi(i)} \notin \mathcal{F}_{B_i}(1-\hat{p}_{i})| P_{i}=\hat{p}_i)$ in Eq. \eqref{eq:calibrationindependence} is aligned with calibrated regressor, it has significant drawbacks in practice. 
%
%First, (C2) still exists and increasing $\hat{p}_{i}$ does not correspond to increasing the localisation performance.
%
%Besides, $\mathbb{P}(b_{\psi(i)} \notin \mathcal{F}_{B_i}(1-\hat{p}_{i})| P_{i}=\hat{p}_i)$ cannot be evaluated on common object detectors, which are not probabilistic, since such detectors directly predict $\hat{b}_i$ and hence $p_{B_i}(b)$ is not available.
%
%Finally, even if the detector is a probabilistic, it is hard to compute due to requiring evaluating a multivariate distribution.
%
%As an example, while $p_{B_i}(b)$ is represented by multivariate Gaussian with full covariance matrix (\cref{sec:relatedwork}) in \cite{RegressionUncOD}, only the diagonal elements of the covariance matrix are used during evaluation\cite{probdet} due to this computation challenge.
%
%Therefore, to discard these drawbacks, we exploit IoU, the common localisation quality, as a proxy for $\mathbb{P}(b_{\psi(i)} \notin \mathcal{F}_{B_i}(1-\hat{p}_{i})| P_{i}=\hat{p}_i)$.
%
%In particular, we use the average IoU of TPs, enabling us to address (C2) since IoU is a higher-better measure aligned with our expectation from $\hat{p}_i$; hence we can now estimate the calibration error for any object detector without a significant computational burden.
%

%we first compute the average calibration error over classes following performance measures in object detection \cite{COCO,LVIS,Objects365,OpenImages, LRPPAMI} to prevent more frequent classes to dominate the calibration error.
%
%Then, we discretize the confidence score space into $J$ equally-spaced bins similar to \cite{calibration,verifiedunccalibration} and split the detections into these bins for each class ($J^{c}=25$ for class $c$) since the underlying integration of $\mathbb{E}_{P_{i}}[\cdot]$ is intractable.
%
%Also, we decouple classification and localisation errors properly by validating the TPs from an IoU of $\tau=0.10$ following the analysis tools of object detectors \cite{Analyzer,TIDE}.
%
%Consequently, the calibration error for a class $c$, denoted by $\mathrm{LaECE}^c$, is given as the weighted average of the differences of the confidence score from the product of precision ($\mathrm{precision}^{c}(j)$) and average IoU of TPs ($\bar{\mathrm{IoU}}^{c}(j)$)
%


{\small
\begin{align}
\label{eq:odcalibrationfinal1}
   \mathrm{LaECE}^c 
   & = \sum_{j=1}^{J^{c}} \frac{|\hat{\mathcal{D}}^{c}_j|}{|\hat{\mathcal{D}}^{c}|} \left\lvert \bar{p}^{c}_{j} - \mathrm{precision}^{c}(j) \times \bar{\mathrm{IoU}}^{c}(j)  \right\rvert,
\end{align}
%
where $\hat{\mathcal{D}}^{c}$ denotes the set of all detections, $\hat{\mathcal{D}}_j^{c}	\subseteq \hat{\mathcal{D}}^{c}$ is the set of detections in bin $j$ and $\bar{p}_{j}^{c}$ is the mean detection scores in bin $j$ for class $c$. 
%
Then, $\mathrm{LaECE}$ of an object detector is the average over $\mathrm{LaECE}^c$ for $c \in \{1, ..., K\}$.
%
%\begin{align}
%\label{eq:mece}
%   \mathrm{mECE} 
%   & = \frac{1}{K} \sum_{c=1}^K \mathrm{ECE}^c.
%\end{align}
%
Thus, we have presented a tractable approach to compute the calibration error accounting for both classification \emph{and} localisation.

1. More frequent classes dominate Eq. \eqref{eq:calibrationindependence}. 
%
Thus, 
%

2. The underlying integration of $\mathbb{E}_{P_{i}}[\cdot]$ is intractable. 
%
Hence, we discretize the confidence score space into $J$ equally-spaced bins similar to \cite{calibration,verifiedunccalibration} and split the detections into these bins for each class ($J^{c}=25$ for class $c$).
%
}
% 3. The term $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i}) | \hat{p}_{i})$ in Eq. \eqref{eq:calibrationindependence} places a higher weighting on localisation due to the mismatch in dimensionality between $B_i$ and $C_i$.
% %
% Furthermore, object detectors, if not probabilistic, directly predict $\hat{b}_i$, and hence $p_{B_i}(b)$ is generally not available.
\begin{figure}[t]
        \captionsetup[subfigure]{}
        \begin{subfigure}[b]{0.25\textwidth}
        \includegraphics[width=\textwidth]{Images/multivariate_approx.pdf}
        \caption{An approximation of IoU}
        \end{subfigure}
        \caption{Blue box: Reference box, on which $\hat{b}_i$ (as the mode of $p_{B_i}(b)$) can be shifted and scaled since IoU is translation- and scale-invariant \cite{BBSampling}. \textbf{(a)} The shape of IoU boundaries. Any top-left and bottom-left point inside a certain locus has at least specified IoU. \textbf{(b)} An example $p_{B_i}(b)$ to approximate IoU boundaries (in red) for top-left corner of the reference box. We use isotropic multivariate log-gamma distribution probability density function in the heatmap. Blue curves at the top and right are the log-gamma distribution for a single dimension.
        }
        \label{fig:iouprob_approx}
\end{figure}

3. Object detectors, if not probabilistic, directly predict $\hat{b}_i$; hence $p_{B_i}(b)$ is generally not available and $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i})| P_{i}=\hat{p}_i)$ cannot be evaluated. 
%
% $B_i$ being four-dimensional and $C_i$ is a univariate, and besides $f_{B_i}(b)$ is mostly not available since the detectors directly predicts $\hat{b}_i$.
%
To address this, we seek an approximation to $\mathbb{P}(b_\psi(i) \in \mathcal{F}_{B_i}(\hat{p}_{i}) | \hat{p}_{i})$ that makes it easy-to-compute for all detectors.
%
To do so, we investigate IoU, which is a common localisation quality, by plotting the boundaries of IoU following \cite{BBSampling}.
%
Fig. \ref{fig:iouprob_approx}(a) suggests that if $p_{B_i}(b)$ is proportional to the IoU boundaries, then IoU follows a function of $\hat{p}_{i}$ implying $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i}) | \hat{p}_{i}) = \mathbb{P}(\mathrm{IoU}(b_{i}, b_{\psi(i)}) > \hat{\mathrm{IoU}} | \hat{p}_{i})$ where $\hat{\mathrm{IoU}}$ is obtained through $\hat{p}_{i}$. 
%
Besides, Fig. \ref{fig:iouprob_approx}(b) depicts that using isotropic multivariate log-gamma distribution as $p_{B_i}(b)$ approximates the IoU boundaries.
%
Having seen their relation, we replace $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i}) | \hat{p}_{i})$ by the average IoU of TPs, enabling us to compute LaECE for all detectors easily.
%
App. \ref{app:subsec_cal_relation} presents the details. 
% When taking the average over all data samples, this reduceds to the average IoU of true positive detections.

Consequently, the calibration error for a class $c$, denoted by $\mathrm{LaECE}^c$, is given as the weighted average of the differences of the confidence score from the product of precision ($\mathrm{precision}^{c}(j)$) and average IoU of TPs ($\bar{\mathrm{IoU}}^{c}(j)$)
%
{\small
\begin{align}
\label{eq:odcalibrationfinal1}
   \mathrm{LaECE}^c 
   & = \sum_{j=1}^{J^{c}} \frac{|\hat{\mathcal{D}}^{c}_j|}{|\hat{\mathcal{D}}^{c}|} \left\lvert \bar{p}^{c}_{j} - \mathrm{precision}^{c}(j) \times \bar{\mathrm{IoU}}^{c}(j)  \right\rvert,
\end{align}}

\normalsize
which, decomposes as the expected error between confidence and average IoU for TP values
\small
\begin{align}
   \label{eq:odcalibrationfinal}
    \mathrm{laECE}^c = \sum_{j=1}^B \frac{|\hat{\mathcal{D}}_j|}{|\hat{\mathcal{D}}|} \left\lvert \bar{p}_{j} - \frac{\sum_{\hat{b}_k \in \hat{\mathcal{D}}_j, \psi(k) > 0,} \mathrm{IoU}(\hat{b}_k, b_{\psi(k)})}{|\hat{\mathcal{D}}_j|}  \right\rvert,
\end{align}

%\normalsize
%
where $\hat{\mathcal{D}}^{c}$ denotes the set of all detections, $\hat{\mathcal{D}}_j^{c}	\subseteq \hat{\mathcal{D}}^{c}$ is the set of detections in bin $j$ and $\bar{p}_{j}^{c}$ is the mean detection scores in bin $j$ for class $c$. 
%
Then, $\mathrm{LaECE}$ of an object detector is the average over $\mathrm{LaECE}^c$ for $c \in \{1, ..., K\}$.
%
%\begin{align}
%\label{eq:mece}
%   \mathrm{mECE} 
%   & = \frac{1}{K} \sum_{c=1}^K \mathrm{ECE}^c.
%\end{align}
%
Thus, we have presented a tractable approach to compute laECE accounting for both classification \emph{and} localisation.
}
%
%In order to decouple classification and localisation errors properly, we follow the analysis tools of object detectors \cite{Analyzer,TIDE} and set the true positive validation threshold as $\tau=0.10$. 
%
%In that case; we prefer LRP Error (Section \ref{sec:relatedwork}) to measure the accuracy over AP, which not only penalizes localisation errors precisely and is more suitable to laECE, as we explore next.
 
%
% Finally, we split the detections as true positives or false positives similar to performance measures; but differently, in order to decouple classification and localisation errors more properly, we set true positive validation threshold as $\tau=0.10$, which is aligned with the error decomposition proposed by the recent analysis tools \cite{Analyzer,TIDE}.
%
% \textbf{Using final detections.}  
%
%\textbf{Using localisation quality in Eq. \ref{eq:calibrationindependence}.} 
%
%As for conventional detectors, while they predict deterministic box coordinates, thereby assuming $\hat{p}_{i}^{loc}=1$ for all $i$; few recent approaches first predict the localisation quality of the detection using an auxiliary head and then obtain the detection confidence score $\hat{p}_{i}$ by multiplying the classification confidence and the predicted localisation quality, which is exactly the case in \ref{eq:score}. As a result, for such detectors $\hat{p}_{i}^{loc}$ corresponds to the output of the auxiliary head predicting the localisation quality. (iii) 
%
% \textbf{Computing localisation calibration error in Eq. \ref{eq:odloccalibration}.} As shown by Kuleshov et al., computing regression calibration error following Eq. \eqref{eq:regressioncalibration} using a cumulative distribution function measures the calibration error of confidence intervals as in Eq. \eqref{eq:odloccalibration}. However, computing multivariate cdf and its inverse is expensive. Accordingly, we follow Harakeh and Waslander \cite{RegressionUncOD} by assuming independence and computing the calibration error following Eq. \eqref{eq:odloccalibration} for four univariate cumulative distributions and report the average calibration error over four dimensions. 
%
% Including cumulative distribution function and its inverse, $\mathbb{P}(b_{\psi(i)} \in \mathcal{F}_{B_i}(\hat{p}_{i})| \hat{p}_{i})$ is time-consuming to compute. For that reason, a recent probabilistic detector \cite{RegressionUncOD} focusing mainly on the calibration in the localisation head and predicting multivariate Gaussian for $f_{B_i}(b)$, preferred ignoring the terms in the covariance except the diagonal to obtain four independent univariate Gaussians. Then, the calibration error is measured as the average of four independent calibration errors based on Eq. \eqref{eq:regressioncalibration}. $\hat{p}_{i}^{loc}$ is not generally available. In terms of probabilistic detectors, existing methods predict the variance of the distribution instead of the confidence score. In such cases, being the output of the object detector, $\hat{p}_{i}$ is still available and Eq. \ref{eq:calibrationindependence} can be obtained; however, Eq. \eqref{eq:odloccalibration} may not be obtained without converting the variance to a confidence score with a range between 0 and 1.
%
% \textbf{Computing calibration errors wrt. detector types.} Note that Eq. \eqref{eq:odcalibrationapprox} can be computed for any detector whether conventional or probabilistic since $\hat{p}_{i}$ has to be included in the detection output. Besides, detection calibration error, we also compute classification and localisation calibration errors for probabilistic object detectors.
%
\begin{figure}[t]
        \captionsetup[subfigure]{}
        \centering
        \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{Images/dummy.pdf}
        \caption{Adding dummy detections}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{Images/threshold.pdf}
        \caption{Effect of thresholding detections}
        \end{subfigure}
        \caption{Red: ATSS, green: F R-CNN, histograms present det/img using right axes, results are on COCO val set with 7.3 objects/img. \textbf{(a)} Dummy detections decrease LaECE (solid line) artificially with no effect on AP (dashed line). LRP Error (dotted line) penalizes dummy detections preventing this trivial way to improve LaECE. \textbf{(b)} AP is maximized with more detections (threshold `none') while LRP Error benefits from properly-thresholded detections.
        %We use LRP-optimal thresholds (not included in the figures) yielding $61.1$ LRP for F R-CNN and $60.2$ LRP for ATSS with around 6 det/img for both, which is comparable to 7.3 objects/image on COCO val set. 
        %
        App. \ref{app:calibration} presents the exact values.
        }
        \label{fig:calibration}
\end{figure}
\blockcomment{
    \begin{table}
        \centering
        \small
        \setlength{\tabcolsep}{0.03em}
        \caption{Adding dummy detections decrease calibration error without affecting performance for AP and oLRP. LRP penalizes the dummy false positives significantly and prevents the laECE to be decreased superficially. However it requires the detections to be thresholded properly (see Table \ref{tab:threshold}). }
        \label{tab:dummydet}
        \begin{tabular}{|c|c|c||c|c|c|c|} \hline
             Detector&Dummy det.&det/img.&$\mathrm{laECE}$&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{LRP}_{0.1}$ \\ \hline
        \multirow{4}{*}{Faster R-CNN}&None&$33.9$&$15.11$&$39.9$&$67.5$&$86.5$\\
        &up to 100&$100$&$3.85$&$39.9$&$67.5$&$96.8$\\
        &up to 300&$300$&$1.37$&$39.9$&$67.5$&$98.8$\\
        &up to 500&$500$&$0.86$&$39.9$&$67.5$&$99.2$\\ \hline
        \multirow{4}{*}{ATSS}&None&$86.4$&$7.69$&$42.8$&$65.7$&$95.1$\\
        &up to 100&$100$&$6.00$&$42.8$&$65.7$&$96.2$\\
        &up to 300&$300$&$1.77$&$42.8$&$65.7$&$98.9$\\
        &up to 500&$500$&$1.09$&$42.8$&$65.7$&$99.3$\\ \hline
        \multirow{4}{*}{RS R-CNN}&None&$100$&$41.90$&$42.0$&$66.0$&$96.0$\\
        &up to 100&$100$&$41.90$&$42.0$&$66.0$&$96.0$\\
        &up to 300&$300$&$11.47$&$42.0$&$66.0$&$98.9$\\
        &up to 500&$500$&$7.02$&$42.8$&$65.7$&$99.3$\\ \hline
        \multirow{4}{*}{D-DETR}&None&$100$&$7.77$&$44.3$&$64.2$&$95.8$\\
        &up to 100&$100$&$7.77$&$44.3$&$64.2$&$95.8$\\
        &up to 300&$300$&$2.18$&$44.3$&$64.2$&$98.9$\\
        &up to 500&$500$&$1.35$&$44.3$&$64.2$&$99.3$\\ \hline
        \end{tabular}
    \end{table}

\begin{table}
    \centering
    \setlength{\tabcolsep}{0.1em}
    \caption{Adding dummy detections decrease calibration error without affecting performance for AP and oLRP. LRP Error penalizes these dummy detections and prevents the laECE to be improved superficially. However it requires the detections to be thresholded properly (see Table \ref{tab:threshold}). }
    \label{tab:dummydet}
    \begin{tabular}{|c|c|c||c|c|c|c|} \hline
         Detector&Dummy det.&det/img.&$\mathrm{laECE}$&$\mathrm{AP}$&$\mathrm{oLRP}$&$\mathrm{LRP}$ \\ \hline
    \multirow{4}{*}{F R-CNN}&None&$33.9$&$15.1$&$39.9$&$67.5$&$86.5$\\
    &up to 100&$100$&$3.9$&$39.9$&$67.5$&$96.8$\\
    &up to 300&$300$&$1.4$&$39.9$&$67.5$&$98.8$\\
    &up to 500&$500$&$0.9$&$39.9$&$67.5$&$99.2$\\ \hline
    \multirow{4}{*}{ATSS}&None&$86.4$&$7.7$&$42.8$&$65.7$&$95.1$\\
    &up to 100&$100$&$6.0$&$42.8$&$65.7$&$96.2$\\
    &up to 300&$300$&$1.8$&$42.8$&$65.7$&$98.9$\\
    &up to 500&$500$&$1.1$&$42.8$&$65.7$&$99.3$\\ \hline
    \end{tabular}
\end{table}

%

\subsection{Localisation-aware ECE [New Narrative]} \label{subsec:mECE}
%
% Here we introduce a core contribution of this work, the Object Detector ECE, termed laECE, which measures the calibration error for object detectors. 
%
Here we derive Localisation-aware ECE in which $\hat{p}_i$, the detection confidence score, accounts for both classification and localisation performance.
%
Before proceeding with our derivation, we note that obtaining $\hat{p}_i$ is still an open problem in object detection.
%
Specifically, while earlier detectors \cite{SSD,FasterRCNN,FocalLoss,RFCN} generally use classification confidence as $\hat{p}_i$, the recent ones \cite{IoUNet,KLLoss,FCOS,GFL,varifocalnet,GFLv2,aLRPLoss,RSLoss,RankDetNet,paa} tend to combine localisation and classification confidences in $\hat{p}_i$, which is shown to be effective for improving the accuracy.
%
To do so, while the methods exploit different approaches, one common example is to train an additional auxiliary head to regress the localisation quality (e.g., IoU) of the predictions \cite{IoUNet,paa,FCOS,ATSS,KLLoss,maskscoring,yolact-plus}, which can be interpreted as the localisation confidence.
%
Then during inference, the predicted classification confidence is combined with the localisation confidence, e.g., through multiplication, so that $\hat{p}_i$ to represent the joint confidence.
%
In our derivation, we adopt this latter perspective, as it aligns with the joint nature of the object detection.

\textbf{Derivation.} We assume a hypothetical object detector, $f_J(X)$, to yield a full joint distribution for each prediction: $f_J(X) = \{p_{C_i, B_i}(c, b)\}^N$ where $p_{C_i, B_i}(c, b)$ is the joint distribution of the random variables $C_i \in \{1, ..., K\}$ and $B_i \in \mathbb{R}^{4}$. 
%
Given $p_{C_i, B_i}(c, b)$, the $i$th detection ($\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$) can be recovered as the modes of the marginal distributions $p_{C_i}(c)$ and $p_{B_i}(b)$, with $\hat{p}_i$ obtained as above.
%
% The mode of the marginal distributions, $p_{C_i}(c)$ and $p_{B_i}(b)$, correspond to $\hat{c}_i$ and $\hat{b}_i$; the detection confidence score $\hat{p}_i$ corresponds to the confidence of the $i$th detection, which is obtained in different ways in practice as aforementioned. 
%
%To represent classification and localisation consistently by $\hat{p}_i$ and address (C1), considering that since $\hat{p}_i$ represents the confidence, not the credible interval, we start with the equivalent criterion for localisation which is $(1-\hat{p}_i)$\% of the ground truths should \textit{not} be within the $\hat{p}_i$ credible interval (compare with calibrated regressor in \cref{fig:iouprob_approx}).
%
%Besides, the probability should match $\hat{p}_i$ not $(1-\hat{p}_i)$; hence we simply rewrite the expression as $\hat{p}_i$\% of the ground truths should not be within the $1-\hat{p}_i$ credible interval.
%hence a higher $\hat{p}_i$ will shrink the credible interval to enforce better localisation performance.
%
Consequently, assuming $\hat{p}_i$ is a realization of the random variable $P_i$, we expect $f_J(X)$ to combine the properties of calibrated classifier and regressor as illustrated in \cref{fig:calibration_def}, hence it is perfectly calibrated if
%
{
\begin{align}\label{eq:gen_calibration}
    \mathbb{P}(C_i = \hat{c}_i, B_i \in \mathcal{B}_i | P_{i} = \hat{p}_i) = \hat{p}_i, \forall \hat{p}_i \in [0, 1],
\end{align}
}
%
such $b_i \in \mathcal{B}_i$ with probability $\hat{p}_i$, implying that if a detection has a confidence of 90\%, then we expect that 90\% of the time the ground truth should lie within an interval around the prediction.
%
However, defining this interval and set is non-trivial.
%
Before proceeding, it is useful highlight the required behaviour of the a calibrated model.
%
In situations where the model is overconfident, we would expect that $\hat{b}_i$ falls in lower density regions of $p_{B_i}(b)$, it is also important to penalise situations where the model may be under-confident, in which case $\hat{b}_i$ will fall in higher density regions.
%



%
For a calibrated model with confidence $\hat{p}_i$, we would expect $\hat{b}_i$ to fall in a density region of $p_{B_i}(b)$ around a point which has a value of  $\hat{p}_i$\% of the modal density.
%
Practically, what we expect is for a confidence of $\hat{p}_i$, then $\hat{p}_i$ of the detections should overlap with the ground truth by a factor of $\hat{p}_i$.
%
Mathematically, it is beneficial to treat 




Expect that the space to overlap with gt space p percent of the time 



%The definition of $\mathcal{B}_i$ relies on the calibration criterion and will be discussed shortly.
%
% $b_{\psi(i)}$ is the ground truth box that $i$th prediction matches with and $\mathcal{F}_{B_i}(\hat{p}_{i})$ is the set of boxes within the $\hat{p}_{i}$ credible region centered at $\hat{b}_i$ in the distribution $p_{B_i}(b)$.
%
%App. \ref{app:calibration} provides the formal definition of $\mathcal{F}_{B_i}(\hat{p}_{i})$.
%
Then, the calibration error of $f_J(X)$ based on Eq. \eqref{eq:gen_calibration} is
%
{
\begin{align}\label{eq:calibration}
    \mathbb{E}_{P_{i}}[ \lvert \hat{p}_{i} - \mathbb{P}(C_i = \hat{c}_i, B_i \in \mathcal{B}_i | P_{i}=\hat{p}_i)) \rvert ],
\end{align}
}
%
% such that $b_{\psi(i)}$ is the ground truth box that $i$th prediction matches and $\mathcal{F}_{B_i}(\hat{p}_{i})$ is the set of boxes within the $1-\hat{p}_{i}$ confidence interval from $\hat{b}_i$ considering $p_{B_i}(b)$\footnote{We use confidence intervals for localisation, which is in fact a regression task, following Kuleshov et al.\cite{regressionunc}. App. \ref{app:subsec_cal_relation} presents the details.}. 
%
where we assume independence between classification and localisation, yielding
%
{
\begin{align}\label{eq:calibrationindependence}
    \mathbb{E}_{P_i}[ \lvert \hat{p}_{i} - \mathbb{P}(C_i = \hat{c}_i | P_{i}=\hat{p}_i) \mathbb{P}(B_i \in \mathcal{B}_i| P_{i}=\hat{p}_{i}) \rvert ].
\end{align}
}
%
%and $\hat{p}_{i}$ can be expressed as, 
%
%\begin{align}\label{eq:score}
%    \hat{p}_{i} = \hat{p}_{i}^{cls} \times \hat{p}_{i}^{loc},
%\end{align}
%
%where $\hat{p}_{i}^{cls}$ and $\hat{p}_{i}^{loc}$ are the confidence scores for classification and localisation respectively. 
%
Note that Eq. \eqref{eq:calibrationindependence} consists of two terms:
%
(i) $\mathbb{P}(C_i = \hat{c}_i | P_{i}=\hat{p}_i)$ is the ratio of the number of correctly-classified detections ($\mathrm{N_{TP}}$) and the total number of detections ($\mathrm{N_{TP}} + \mathrm{N_{FP}}$), which is simply the precision.
%
(ii) $\mathbb{P}(B_i \in \mathcal{B}_i| P_{i}=\hat{p}_{i})$ determines the calibration of the localisation prediction, which we investigate further next.
%

\textbf{A suitable choice of regression calibration criterion.} 
%
We observed there are two main set of approaches to measure the calibration error of a probabilistic regressor.
%
The first set of measures aims to align the predicted and empirical cumulative distribution functions \cite{regressionunc,distributioncalibrationregression}, implying $p\%$ credible interval from the mode of the predictive distribution should include $p\%$ of the ground truths for $p \in [0,1]$. 
%
In this case, $\mathcal{B}_i$ represents the bounding boxes within $\hat{p}_{i}$ credible region of $\hat{b}_i$ in $p_{B_i}(b)$ (App. \ref{app:calibration} provides the formal definition).
%
However, this approach does not fit into our purpose as it does not account for the confidence scores $\hat{p}_{i}$ as intended, i.e. as $\hat{p}_{i}$ increases, $\mathcal{B}_i$ enlarges and cover more bounding boxes, instead of shrinking to ensure a higher localisation quality. 
%
In the extreme case, when $\hat{p}_{i}=1$, the credible region spans across the entire $p_{B_i}(b)$ implying $\mathbb{P}(B_i \in \mathcal{B}_i| P_{i}=\hat{p}_{i})=1$; thereby ignoring the localisation quality of the prediction $\hat{b}_i$.
%
The second set of measures considers the discrepancy between the uncertainty (or confidence) and the regression error (or accuracy) \cite{UCE,UCE2}.
%
To illustrate, UCE \cite{UCE} aims to align the variance of the predictive distribution with the mean squared error of the mode of the prediction.
%
Accordingly, considering that $\hat{p}_i$ should reflect the joint quality of the prediction to enable the subsequent systems to decide properly, this perspective corresponds to using a higher-better performance measure as a proxy for $\mathbb{P}(B_i \in \mathcal{B}_i| P_{i}=\hat{p}_{i})$ in Eq. \eqref{eq:calibrationindependence}.
%
With such a proxy, the higher precision or localisation quality of a prediction is, the higher $\hat{p}_i$ should be, such that the error in Eq. \eqref{eq:calibrationindependence} is minimized, which is intuitive.
%
In particular, we use the average IoU of TPs, enabling us to estimate the calibration error of any object detector only by relying on the conventional representation of the detections ($\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$).

\textbf{Practical Usage.} We compute the average calibration error over classes following performance measures in object detection \cite{COCO,LVIS,Objects365,OpenImages, LRPPAMI} to prevent more frequent classes to dominate the calibration error; and discretize the confidence score space into $J$ equally-spaced bins by splitting the detections into these bins for each class ($J^{c}=25$ for class $c$) similar to \cite{calibration,verifiedunccalibration}.
%
Consequently, the calibration error for a class $c$, denoted by $\mathrm{LaECE}^c$, is given as the weighted average of the differences of the confidence score from the product of precision ($\mathrm{precision}^{c}(j)$) and average IoU of TPs ($\bar{\mathrm{IoU}}^{c}(j)$)
%
{\small
\begin{align}
\label{eq:odcalibrationfinal1}
   \mathrm{LaECE}^c 
   & = \sum_{j=1}^{J^{c}} \frac{|\hat{\mathcal{D}}^{c}_j|}{|\hat{\mathcal{D}}^{c}|} \left\lvert \bar{p}^{c}_{j} - \mathrm{precision}^{c}(j) \times \bar{\mathrm{IoU}}^{c}(j)  \right\rvert,
\end{align}}
%
where $\hat{\mathcal{D}}^{c}$ denotes the set of all detections, $\hat{\mathcal{D}}_j^{c}	\subseteq \hat{\mathcal{D}}^{c}$ is the set of detections in bin $j$ and $\bar{p}_{j}^{c}$ is the average of the detection confidence scores in bin $j$ for class $c$. 
%
Then, $\mathrm{LaECE}$ of an object detector is the average over $\mathrm{LaECE}^c$ for $c \in \{1, ..., K\}$.
%
Thus, we have presented a tractable approach to compute the calibration error of object detectors accounting for both classification \emph{and} localisation.
}

\blockcomment{
%
{
\begin{align}\label{eq:gen_calibration_}
    \mathbb{P}(C_i = \hat{c}_i, B_i \in \mathcal{B}(\hat{p}_i) | P_{i} = \hat{p}_i) = \hat{p}_i, \forall \hat{p}_i \in [0, 1],
\end{align}
}
%
%such that $\mathcal{B}_i$ is the set of bounding boxes that ensures the marginal distribution for localisation $p_{B_i}(b)$ to be calibrated based on a criterion and will be discussed soon.
%
%The definition of $\mathcal{B}_i$ relies on the calibration criterion and will be discussed shortly.
%
% $b_{\psi(i)}$ is the ground truth box that $i$th prediction matches with and $\mathcal{F}_{B_i}(\hat{p}_{i})$ is the set of boxes within the $\hat{p}_{i}$ credible region centered at $\hat{b}_i$ in the distribution $p_{B_i}(b)$.
%
%App. \ref{app:calibration} provides the formal definition of $\mathcal{F}_{B_i}(\hat{p}_{i})$.
%
with the calibration error of
%
{
\begin{align}\label{eq:calibration}
    \mathbb{E}_{P_{i}}[ \lvert \hat{p}_{i} - \mathbb{P}(C_i = \hat{c}_i, B_i \in \mathcal{B}(\hat{p}_i) | P_{i}=\hat{p}_i)) \rvert ],
\end{align}
}
%
% such that $b_{\psi(i)}$ is the ground truth box that $i$th prediction matches and $\mathcal{F}_{B_i}(\hat{p}_{i})$ is the set of boxes within the $1-\hat{p}_{i}$ confidence interval from $\hat{b}_i$ considering $p_{B_i}(b)$\footnote{We use confidence intervals for localisation, which is in fact a regression task, following Kuleshov et al.\cite{regressionunc}. App. \ref{app:subsec_cal_relation} presents the details.}. 
%
where we assume independence between classification and localisation, yielding
%
{
\begin{align}\label{eq:calibrationindependence_}
    \mathbb{E}_{P_i}[ \lvert \hat{p}_{i} - \mathbb{P}(C_i = \hat{c}_i | P_{i}=\hat{p}_i) \mathbb{P}(B_i \in \mathcal{B}(\hat{p}_i)| P_{i}=\hat{p}_{i}) \rvert ].
\end{align}
}
}

\blockcomment{
\textbf{A suitable choice of regression calibration criterion.} 
%
We observed there are two main set of approaches to measure the calibration error of a probabilistic regressor.
%
The first set of measures aims to align the predicted and empirical cumulative distribution functions \cite{regressionunc,distributioncalibrationregression}, implying $p\%$ credible interval from the mode of the predictive distribution should include $p\%$ of the ground truths for $p \in [0,1]$. 
%
In this case, $\mathcal{B}_i$ represents the bounding boxes within $\hat{p}_{i}$ credible region of $\hat{b}_i$ in $p_{B_i}(b)$ (App. \ref{app:calibration} provides the formal definition).
%
However, this approach does not fit into our purpose as it does not account for the confidence scores $\hat{p}_{i}$ as intended, i.e. as $\hat{p}_{i}$ increases, $\mathcal{B}_i$ enlarges and cover more bounding boxes, instead of shrinking to ensure a higher localisation quality. 
%
In the extreme case, when $\hat{p}_{i}=1$, the credible region spans across the entire $p_{B_i}(b)$ implying $\mathbb{P}(B_i \in \mathcal{B}_i| P_{i}=\hat{p}_{i})=1$; thereby ignoring the localisation quality of the prediction $\hat{b}_i$.
%
The second set of measures considers the discrepancy between the uncertainty (or confidence) and the regression error (or accuracy) \cite{UCE,UCE2}.
%
To illustrate, UCE \cite{UCE} aims to align the variance of the predictive distribution with the mean squared error of the mode of the prediction.
%
Accordingly, considering that $\hat{p}_i$ should reflect the joint quality of the prediction to enable the subsequent systems to decide properly, this perspective corresponds to using a higher-better performance measure as a proxy for $\mathbb{P}(B_i \in \mathcal{B}_i| P_{i}=\hat{p}_{i})$ in Eq. \eqref{eq:calibrationindependence_}.
%
With such a proxy, the higher precision or localisation quality of a prediction is, the higher $\hat{p}_i$ should be, such that the error in Eq. \eqref{eq:calibrationindependence_} is minimized, which is intuitive.
%
In particular, we use the average IoU of TPs, enabling us to estimate the calibration error of any object detector only by relying on the conventional representation of the detections ($\{\hat{c}_i, \hat{b}_i, \hat{p}_i\}$).
}
